FIMP-HGA: A Novel Approach to Addressing the Partitioning Min-Max Weighted Matching Problem

The Partitioning Min-Max Weighted Matching (PMMWM) problem, being a practical NP-hard problem, integrates the task of partitioning the vertices of a bipartite graph into disjoint sets of limited size with the classical Maximum-Weight Perfect Matching (MPWM) problem. Initially introduced in 2015, the state-of-the-art method for addressing PMMWM is the MP$_{\text{LS}}$. In this paper, we present a novel approach, the Fast Iterative Match-Partition Hybrid Genetic Algorithm (FIMP-HGA), for addressing PMMWM. Similar to MP$_{\text{LS}}$, FIMP-HGA divides the solving into match and partition stages, iteratively refining the solution. In the match stage, we propose the KM-M algorithm, which reduces matching complexity through incremental adjustments, significantly enhancing runtime efficiency. For the partition stage, we introduce a Hybrid Genetic Algorithm (HGA) incorporating an elite strategy and design a Greedy Partition Crossover (GPX) operator alongside a Multilevel Local Search (MLS) to optimize individuals in the population. Population initialization employs various methods, including the multi-way Karmarkar-Karp (KK) algorithm, ensuring both quality and diversity. At each iteration, the bipartite graph is adjusted based on the current solution, aiming for continuous improvement. To conduct comprehensive experiments, we develop a new instance generation method compatible with existing approaches, resulting in four benchmark groups. Extensive experiments evaluate various algorithm modules, accurately assessing each module's impact on improvement. Evaluation results on our benchmarks demonstrate that the proposed FIMP-HGA significantly enhances solution quality compared to MP$_{\text{LS}}$, meanwhile reducing runtime by 3 to 20 times.

==> 01-IntroOLD.tex <==
\IEEEPARstart{I}{n}  this paper, we consider the Partitioning Min-Max Weighted Matching (PMMWM) problem proposed by \cite{a1}. The PMMWM is defined by a weighted bipartite graph $G(U,V,E)$ with disjoint vertex sets $U$, $V$ and edge set $E = \{e_{uv}|u \in U, v \in V\}$, where $U$ needs to be partitioned into $m$ disjoint partitions with no more than $\bar{u}$ vertices each. Given a maximum matching on $G$, the weight of a partition is defined as the sum of the edge weights for the edges matching the vertices in the partition. The goal of the problem is to find a matching and a partition to minimize the largest weight of the partitions. The PMMWM is an NP-hard problem in the strong sense.

\begin{figure}[H]
\centering
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{Figure/example.png}
  \caption{A feasible solution}
  \label{fig:example1}
\end{subfigure}\hfil
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{Figure/example-better.png}
  \caption{An improved solution}
  \label{fig:example2}
\end{subfigure}
\caption{A PMMWM example.}
\label{fig:pmmwm}
\end{figure}

\rfig{example1} illustrates a feasible solution to a PMMWM instance. The colored edges indicate the maximum matching edges and the associated weights are marked beside. The left part of the bipartite graph, $U=\{u_1,u_2,...,u_6\}$, is divided into three partitions, $U_1$, $U_2$ and $U_3$ labeled with different colors. The weights of the three partitions are 4, 2 and 5. The value of the objective function is 5. 

We consider two different ways to optimize the objective function.
The first is to modify the partition strategy. We can move $u_6$ to $U_2$, then the weights of the three partitions become 4, 3, and 4. The objective function value is 4. 
The second is to modify the matching strategy. For $u_3,u_5$, if we replace the current matching edges $e_{u_3 v_6}, e_{u_5 v_2}$ with edges $e_{u_3 v_2},e_{u_5 v_6}$, then the weights of the partitions become 4, 4, 4, as shown in \rfig{example2}. Although the total weight of the matching edges is increased, the final objective function is reduced to 4.

\citeauthor{a1} show an application of the PMMWM at small to medium sized seaports. The seaports include long-term storage areas and temporary storage areas. The vertex set $U$ denotes the empty slots in the long-term storage area, the vertex set $V$ denotes the containers in the temporary storage area, and the edge weight $c_{uv}$ for an edge $e_{uv} \in E$ denotes the cost required to move the container $v$ to the empty slot $u$. The parameter $m$ indicates the number of available telescopic stackers and $\bar{u}$ indicates the upper limit of the number of containers that can be handled by one telescopic stacker. Suppose the cost of a telescopic stacker equals to the total cost of moving its containers, the goal of the problem is to minimize the maximum cost among the telescopic stackers.
%the cost of the telescopic stacker with the maximum cost.

We find another application of the PMMWM that is related to the task allocation. Suppose there are $n$ workers, $n$ tasks, and $m$ machines in a workshop. Each task should be performed on a machine by a worker, each worker performs only one task, and each machine can take at most one task at a time. The vertex set $U$ denotes the workers, $V$ denotes the tasks, and the edge weight $c_{uv}$ denotes the spending time of performing task $v$ by worker $u$. The parameter $\bar{u}$ indicates the maximum number of tasks that can be performed by each machine per day (working period). The goal of the problem is to determine the matching between workers and tasks, and the partition of workers to machines, so as to minimize the longest spending time among the machines. % of the machine with the longest spending time.

% [TODO] more work
% 提出了一个新框架叫Fast Matching Partition，他在Matching Partition的基础上。
% 在Partiton阶段，在不改变复杂度的前提下，使用Karmarkar-Karp算法生成初始解，

% 我们总结了MPLS算法的两个缺点，并针对这两个方面提出改进方案：（1）matching阶段效率较低（2）partition阶段优度较低
In this work, we analyze the MP$_{\text{LS}}$ algorithm proposed by \cite{a1}. It solves this problem by Matching-Partition(MP) framework, which employs the KM algorithm for matching phase and applies a local search strategy for partition phase. As follows, we find two main weakness of the MP$_{\text{LS}}$ algorithm and propose improvement strategies for these two aspects:

(1) MP$_{\text{LS}}$ is an iterative algorithm, and at each iteration it adjusts the edge weight matrix of the bipartite graph to generate a different initial maximum matching by an exact algorithm. In the matching phase,MP$_{\text{LS}}$ applies a complete matching algorithm to the bipartite graph each iteration, which becomes a time bottleneck. However,  the modified bipartite graph does not change much at each iteration, there are many redundant operations that can be optimized. 
% 因此，我们提出了KM-M算法替换MP框架中每轮匹配使用的KM算法，得到更高效的框架FMP
Hence, we propose the KM-M algorithm to replace the KM algorithm used in each round of matching within the MP framework, resulting the efficent Fast Matching-Parition(FMP) framework, which reuses the matching results of the edges that their weights are not changed in the last iteration, and hence reduces the time complexity from $O(n^3)$ to $O(n^2)$ of the matching phase while maintaining the resulting quality.

(2) In the partition phase, the initial solution algorithm of MP$_{\text{LS}}$ primarily emphasizes efficiency, but there is still considerable room for improvement in the quality of the solution. The subsequent local search algorithm only considers simple exchange actions and neglects diversity, making it susceptible to falling into local optima and directly affecting the quality of the solution. In this paper, we employs the multi-way Karmarkar-Karp algorithm for the K-way number partition problem to generate higher-quality initial solutions. Following this, we proposed a efficient two-level local search strategy to enhance the quality of the solution called Improved Local Search(ILS). Initially, It attempts to enhance the solution's quality through a certain extent of search(first level). If these actions fail to yield improvements, the strategy then shifts to a more fine-grained search approach(second level). 
Furthermore, we propose a hybrid evolution strategy and corresponding crossover operators to ensure the diversity of the algorithm. Each solution obtained through crossover is optimized by the ILS algorithm. To accelerate the evolution of the population, we propose the concept of elite individuals.

% In this work, we analyze the MP$_{\text{LS}}$ algorithm proposed by \cite{a1} and find that the time bottleneck is in the matching phase. MP$_{\text{LS}}$ is an iterative algorithm, and at each iteration it adjusts the edge weight matrix of the bipartite graph to generate a different initial maximum matching by an exact algorithm. Since the modified bipartite graph does not change much at each iteration, there are many redundant operations that can be optimized. 
% Hence, we propose a new framework called Fast Matching-Partition(FMP), which reuses the matching results of the edges that their weights are not changed in the last iteration, and hence reduces the time complexity from $O(n^3)$ to $O(n^2)$ of the matching phase while maintaining the resulting quality.

% MP_LS分为多轮迭代，每轮迭代只调整一条边的权重，但是却要对整个图重新进行带权二分图匹配。除第一轮外，每次重新匹配都包含大量的重复操作，大大增加了时间开销。
% MP$_{\text{LS}}$ involves multiple rounds of iteration, where each round adjusts the weight of a single edge while performing weighted bipartite graph matching on the entire graph. However, in each round after the first one, the re-matching process involves significant redundant operations, leading to a substantial increase in time complexity.
% 本文提出了Fast Matching-Partition框架，在KM算法的基础上提出了用于解决对原带权二分图进行增量修改的KM-M算法。在保证理论最优的前提下，大幅度提升时间效率。
% This article introduces the Fast Matching-Partition framework, which proposes the KM-M algorithm based on the KM algorithm to solve incrementally modified weighted bipartite graphs. By ensuring theoretical optimality, the proposed approach significantly improves time efficiency.

% 在Partition阶段，MPLS的初始解算法主要考虑了效率，在优度上仍有很大的优化空间。后续的局部搜索算法只考虑了简单的交换动作，没有关注算法的多样性，很容易陷入局部最优，直接影响解的优度。
%In the Partition phase, the initial solution algorithm of MPLS primarily emphasizes efficiency, but there is still considerable room for optimization in terms of solution quality. The subsequent local search algorithm only considers simple exchange actions and neglects the algorithm's diversity, making it susceptible to falling into local optima and directly affecting the quality of the solution.
% 本文使用了用于K-way number partition问题中的Karmarkar-Karp算法，能生成质量更高的初始解。
% 在改进初始解阶段，提出了二级局部搜索策略。其将领域动作
% 最后，为了保证算法的多样性，本文引入了种群进化的策略，提出了相应的交叉算符。为了防止运行效率过慢，引入了精英个体的概念加速种群的进化过程。

% 另外，对数据集分析后，我们按二分图的疏散性和密度对数据进行分类。按这种方式对之前提出的数据集进行整理以及补充，使得能对算法进行更全面的实验及分析。
Additionally, after analyzing the dataset, we classify the data based on the sparsity and density of the bipartite graph. By organizing and supplementing the datasets previously proposed in this way, we enable a more comprehensive experimentation and analysis of the algorithm.

The remainder of the paper is organized as follows.
Section 2 introduces a detailed formulation of the PMMWM problem. Subsequently, Section 3 explores related works and succinctly introduces the MP$_{\text{LS}}$ algorithm. In Section 4, we provide an in-depth description of the KMP framework, along with a validation of its correctness. Section 5 focuses on the techniques utilized in the matching phase. The process of dataset generation and the corresponding test results are detailed in Section 6. Finally, Section 7 summarizes the main conclusions of this paper.
% 第四章详细描述了KMP框架以及证明其正确性，第五章详细描述了匹配阶段使用的技巧。第六章描述了数据集的生成方式以及测试结果
 % We describe the related works in Section 2, and formulate the PMMWM problem in Section 3. Section 4 briefly introduces the MP$_{\text{LS}}$ algorithm, and Section 5 details the proposed MP$_{\text{KM-M}}$ algorithm and proves the correctness. Section 6 reports the results of the experiment, and Section 7  summarizes the main conclusion of this paper.


 % [TODO] 是否需要分段



==> 02-Prob.tex <==
Let $G(U,V,E)$ be a weighted bipartite graph, where $U$ and $V$ are two disjoint vertex sets, and $E = \{e_{uv}|u \in U, v \in V\}$ denotes the set of pairwise edges. 
Assume $|U| = n_1$, $|V| = n_2$, and $n_1 \leq n_2$. Each edge $e_{uv} \in E$ is associated with a weight $c_{uv}\in\mathbb{Q}^{+}_{0}$. Define a matching as the set $M\subseteq E$ of pairwise nonadjacent edges, and the maximum matching~\citep{DBLP:journals/computing/DerigsZ78} as the matching with the largest $|M|$ among all matchings on $G$. 

%Let $G(U,V,E)$ be a weighted bipartite graph. The vertices of $U$ and $V$ are indexed by $i=1,...,n_{1}$ and $j=1,...,n_{2}$, respectively, assuming $n_{1}\le n_{2}$. The weight $c(e)=c_{uv}\in\mathbb{Q}^{+}_{0}$ is associated with each edge of $G$. Define a matching as the set $M\subseteq E$ of pairwise nonadjacent edges and the maximum matching\cite{DBLP:journals/computing/DerigsZ78} as the matching with the largest $|M|$ among all matchings on $G$. 

Assume that for any given weighted bipartite graph, there exists at least one maximum matching $\Pi$ such that $|\Pi|=n_{1}$. Define a partition $\mathcal{P}$ of $U$ that divides $U$ into $m$ disjoint partitions $U_1,U_2,...,U_m$, with at most $\bar{u}$ vertices in each partition. The goal of the PMMWM is to find a partition $\mathcal{P}$ of $U$ and a maximum matching $\Pi$ of $G$ that minimizes the evaluation function $f(\mathcal{P}, \Pi) := \max_{k\in\{1, ...,m\}}\{\sum_{u\in U_k,(u,v)\in\Pi}c_{uv}\}$.


%Assume that for any given weighted bipartite graph, there exists a maximum matching $\Pi$ such that $|\Pi|=n_{1}$, and assume that $U$ is assigned into $m$ disjoint partitions $U_1,U_2,...,U_m$, with at most $\bar{u}$ vertices in each partition, the value of the maximum matching $\Pi$ is defined as $w(\Pi):=\max_{k\in\{1, ...,m\}}\{\sum_{u\in U_k,(u,v)\in\Pi}c_{uv}\}$.

%Based on the above assumptions, the PMMWM can be defined as follows: assigning the vertex set $U$ into $m$ possibly empty disjoint partitions $U_1,U_2,...,U_m$ with at most $\bar{u}$ vertices in each partition, and find a maximum matching $\Pi$ on $G$ such that the value of $\Pi$ is the smallest among all possible assignment of $U$.

Let $z_{uvk}$ be a binary variable such that $z_{uvk} = 1$ if $u \in U_k, e_{uv} \in \Pi$, and $z_{uvk} = 0$ otherwise. 
%The mathematical model of the PMMWM is as follows.
The PMMWM problem can be formalized as follows. 

\begin{equation*}
\begin{aligned}
    \label{eq:pmmwm}
    & \min_{\mathbf{z}} \max_{k\in\{1,…,m\}} \{\sum_{u\in U}\sum_{v\in V}c_{uv}z_{uvk}\} \\
    %\label{eq:pmmwm_1}
\text{s.t.} \qquad & (1) \qquad\sum_{k=1}^{m}\sum_{v\in V}z_{uvk}=1\quad\forall u\in U,\\
    &(2) \qquad \sum_{k=1}^{m}\sum_{u\in U}z_{uvk}\le1\quad\forall v \in V,\\
    &(3) \qquad \sum_{k=1}^{m}z_{uvk}=1\quad\forall e_{uv} \in E,\\
    &(4) \qquad \sum_{u \in U}\sum_{v\in V}z_{uvk}\le\bar{u}\quad\forall k\in\{1,…,m\}.
\end{aligned}
\end{equation*}


\iffalse
\begin{equation}
    \label{eq:pmmwm_2}
    (2) \qquad \sum_{k=1}^{m}\sum_{u\in U}z_{uvk}\le1\quad\forall v \in V,
\end{equation}
    
\begin{equation}
    \label{eq:pmmwm_3}
    (3) \qquad \sum_{k=1}^{m}z_{uvk}=1\quad \forall u\in U, v \in V,
\end{equation}
    
\begin{equation}
    \label{eq:pmmwm_4}
    (4) \qquad \sum_{u \in U}\sum_{v\in V}z_{uvk}\le\bar{u}\quad\forall k\in\{1,…,m\}.
\end{equation}
\fi


The objective function minimizes the maximum matching weight among all possible assignments and maximum matchings. Constraints (1) and (2) are the well-known constraints on the maximum matching. Constraint (3) forces each vertex $u\in U$ to belong to exactly one partition $U_k,k\in \{1,...,m\}$. Constraint (4) restricts that the size of the partition does not exceed $\bar{u}$. %\eqref{eq:pmmwm_5} and \eqref{eq:pmmwm_6} are the domains of the variables.

\iffalse

Define the following binary variables

\begin{equation}
    x_{ij}:=\begin{cases}
    1\quad\text{if }(i,j)\in\Pi,\\
    0\quad\text{else},
    \end{cases} \forall(i,j)\in E
\end{equation}
    
\begin{equation}
    y_{ik}:=\begin{cases}
    1\quad\text{if }i\in U_k,\\
    0\quad\text{else,}
    \end{cases} \forall i\in U,k\in \{1,…,m\}.
\end{equation}

The nonlinear mathematical model of the PMMWM is as follows.

\begin{equation}
    \label{eq:pmmwm}
    \min_{\mathbf{x,y}} \max_{k\in\{1,…,m\}}\{\sum_{i\in U}\sum_{j\in V}c_{ij}y_{ik}x_{ij}\}
\end{equation}
    
\begin{equation}
    \label{eq:pmmwm_1}
    \text{s.t.}\qquad\sum_{j\in V}x_{ij}=1\quad\forall i\in U,
\end{equation}
    
\begin{equation}
    \label{eq:pmmwm_2}
    \sum_{i\in U}x_{ij}\le1\quad\forall j \in V,
\end{equation}
    
\begin{equation}
    \label{eq:pmmwm_3}
    \sum_{k=1}^{m}y_{ik}=1\quad\forall i\in U,
\end{equation}
    
\begin{equation}
    \label{eq:pmmwm_4}
    \sum_{i\in U}y_{ik}\le\bar{u}\quad\forall k\in\{1,…,m\},
\end{equation}
    
\begin{equation}
    \label{eq:pmmwm_5}
    x_{ij}\in\{0,1\}\quad\forall(i,j)\in E,
\end{equation}
    
\begin{equation}
    \label{eq:pmmwm_6}
    y_{ik}\in\{0,1\}\quad\forall i\in U,k\in\{1,…,m\}.
\end{equation}

The objective function \eqref{eq:pmmwm} minimizes the maximum matching weight among all possible assignment. \eqref{eq:pmmwm_1} and \eqref{eq:pmmwm_2} are the constraints on the maximum matching. \eqref{eq:pmmwm_3} forces each vertex $u\in U$ to belong to and only belong to one partition $U_k,k\in 1,...,m$. \eqref{eq:pmmwm_4} restricts the size of the partition does not exceed $\bar{u}$. \eqref{eq:pmmwm_5} and \eqref{eq:pmmwm_6} are the domains of the variables.

By introducing additional variables $z_{ijk}\ge0$ for all $i\in U,j\in V,k\in\{1,...,m\}$, the model can be linearized.

\begin{equation}
    \min_{\mathbf{x,y}}c
\end{equation}
    
\begin{equation}
    \text{s.t. constraints}\eqref{eq:pmmwm}-\eqref{eq:pmmwm_6},
\end{equation}
    
\begin{equation}
    c\ge\sum_{i\in U}\sum_{j\in V}c_{ij}z_{ijk}\quad\forall k \in\{1,…,m\},
\end{equation}
    
\begin{equation}
    z_{ijk}\ge y_{ik}+x_{ij}-1\quad\forall i\in U,j\in V,k\in\{1,…,m\},
\end{equation}
    
\begin{equation}
    z_{ijk}\ge 0\quad\forall i\in U,j\in V,k\in\{1,…,m\}.
\end{equation}

\fi


==> 03-RW.tex <==
The PMMWM is an extension problem of the Min-Max Weighted Matching (MMWM) problem~\citep{a2}. MMWM is motivated by the container transshipment in a rail-road terminal. MMWM has the same objective function as PMMWM, but the partitioning of the vertices is given. So, MMWM only needs to decide the matching result. \cite{a2} prove that the MMWM is NP-hard in the strong sense and develop heuristics to find the matching that the average gap to the optimal solution is less than 1\%. %one percentage. 

When there is only one partition (i.e., $m = 1$), the PMMWM can be reduced to an assignment problem that just needs to find a maximum matching with minimum weight. For the assignment problem, \cite{a3} propose an exact polynomial-time algorithm called the Hungarian method which is also denoted as the KM algorithm. The KM algorithm is applied on the matching process of both MP$_{\text{LS}}$~\citep{a1} and MP$_{\text{KM-M}}$. Moreover, the KM algorithm inspired \cite{primal-dual} to propose the primal-dual method for linear programming, which is widely used for various combinatorial optimization problems. In this paper, we also use the primal-dual method to prove the correctness of the proposed MP$_{\text{KM-M}}$ algorithm. 

However, in some practical applications, the partition also needs to be determined, for instance in the small to medium sized seaports where containers are handled by reach stackers. So, \cite{a1} propose the PMMWM and decompose the problem into two stages, matching and partitioning, and solve them either exactly or heuristically. They propose two different heuristic frameworks with different order of the matching and partitioning phases. For the partitioning-matching framework, they propose two heuristics called PM$_{\text{BPS}}$ and PM$_{\text{REG}}$. For the matching-partitioning framework, they propose other two heuristics called MP and MP$_{\text{LS}}$. By performing extensive experiments, \cite{a1} conclude that the MP$_{\text{LS}}$ algorithm is the best-performing one among the four algorithms, and is also robust against changes in the graph structure.


\cite{7376822} also apply PMMWM to the intermodal transport, and propose a heuristic based on tabu search~\citep{DBLP:journals/informs/Glover89,DBLP:journals/informs/Glover90} and a genetic algorithm~\citep{DBLP:books/daglib/0019083}. They propose three neighborhood structures for the tabu search heuristic and a crossover operator for the genetic algorithm. But these two algorithms are not as effective as the MP$_{\text{LS}}$ algorithm. Therefore, MP$_{\text{LS}}$ is still the best-performing algorithm for the PMMWM. 
In this work, we select MP$_{\text{LS}}$ as the baseline algorithm, and our proposed MP$_{\text{KM-M}}$ algorithm significantly outperforms MP$_{\text{LS}}$ on the algorithm efficiency while keeping the same effectiveness.

\subsection{MP$_{\text{LS}}$ Algorithm}
\input{03.01-MPLS}

% intro里面对weakness的描述用不用放在这里


==> 03.01-MPLS.tex <==
The MP$_{\text{LS}}$ algorithm~\citep{a1} decomposes the PMMWM problem into two components, i.e., matching and partition. 
% 下文中称为MP框架
Referred to as the MP framework in the following text.
MP$_{\text{LS}}$ is an iterative heuristic algorithm, and each iteration consists of three stages. The first stage generates a maximum matching $\Pi$ of $G = (U,V,E)$, and the second stage calculates a partition $\mathcal{P}$ of $U$ that satisfies constraints (3) and (4) of the problem. Then the combination of $\mathcal{P}$ and $\Pi$ results in a feasible solution for an input instance. In the third stage, MP$_{\text{LS}}$ makes a slight adjustment on the weight matrix of $E$ and then returns to the first stage of the next iteration, which can help the algorithm to escape from the local optima and find better solutions. We denote $G'$ to be the bipartite graph where the edge weight matrix is adjusted. Starting from $G' = G$, the MP$_{\text{LS}}$ algorithm repeats the three stages until a termination condition is met. Implementation details of the three stages are as follows.

In the first stage, MP$_{\text{LS}}$ applies the KM algorithm~\citep{DBLP:books/daglib/p/Kuhn10} to obtain a minimum weight maximum matching $\Pi$ of the bipartite graph $G'$. %The minimum weight maximum matching 
So match $\Pi$ is a maximum matching such that the total weight of the edges belonging to the matching is minimized.

In the second stage, MP$_{\text{LS}}$ first assumes the maximum matching $\Pi$ of $G'$ is fixed, then the problem can be regarded as a restricted partitioning problem of $U$, by setting the weight of each vertex $u \in U$ to $w_u = c_{uv}, e_{uv} \in \Pi$ (note that when calculating the partition in this stage, $c_{uv}$ is always the original weight of edge $e_{uv}$). MP$_{\text{LS}}$ uses the RPH~\citep{a2} heuristic algorithm to solve the restricted partitioning problem and obtains a feasible solution to the PMMWM.
% 首先生成一个初始解，然后再用局部搜索进行优化
An initial solution is first generated and then optimized with a local search


In the third stage, MP$_{\text{LS}}$ changes the weight of one edge in $G'$ so as to adjust the bipartite matching solution in the next iteration. Let $k = \mathop{\arg\max_{k \in \{1,...,m\}}{\{\sum_{u \in U_k, e_{uv} \in \Pi}{c_{uv}}\}}}$, then the selected edge $e \in \Pi$ is an edge with the maximum weight among the current edges of $\Pi$ that are incident to vertices of component $U_k$. MP$_{\text{LS}}$ changes the weight of $e$ in $G'$ to a large value ($10^2 c_{\max}$ in default, where $c_{\max}$ is the maximum edge weight in the input graph) to largely reduce the probability that this edge will belong to the matching calculated in the first stage of the next iteration. %, and returns to the first stage.

The MP$_{\text{LS}}$ algorithm stops when the solution to the PMMWM has not improved for 20 iterations.

==> 04-FMP.tex <==
In this section, we propose an FMP framework that significantly improves the efficiency of the SOTA algorithm, MP$_{\text{LS}}$, for solving the PMMWM. 
We observe that in each iteration, MP framework only changes the weight of one edge in the third stage, but recalculates the minimum weight maximum matching of the whole graph in the first stage of the next iteration, which is redundant and very time-consuming. 
Specifically, the KM algorithm used in the first stage of MP$_{\text{LS}}$ will cost $O(n^3)$ time in each iteration. To handle this issue, the proposed KM-M algorithm optimizes the efficiency of the first stage by simplifying the matching process.
%我们称将MP框架中用于匹配的KM算法替换为KM-M算法的框架为FMP
We refer to the framework where the KM algorithm used for matching in the MP framework is replaced with the KM-M algorithm as FMP.

This section first introduce the KM algorithm in detail, then presents the simplified matching algorithm KM-M in the proposed FMP framework and the main process of it, and finally provides the proof on the correctness of the KM-M algorithm.


%In this section, we propose an MP$_{\text{KM-M}}$ algorithm that significantly improves the efficiency of the SOTA algorithm, MP$_{\text{LS}}$, for solving the PMMWM. 
%We observe that in each iteration, MP$_{\text{LS}}$ only changes the weight of one edge in the third stage, but recalculates the minimum weight maximum matching of the whole graph in the first stage of the next iteration, which is redundant and very time-consuming. 
%Specifically, the KM algorithm used in the first stage of MP$_{\text{LS}}$ will cost $O(n^3)$ time in each iteration. To handle this issue, the proposed MP$_{\text{KM-M}}$ optimizes the efficiency of the first stage by simplifying the matching process.

\subsection{The KM Algorithm}
\input{04.01-KM}

\subsection{The Simplified KM-M Matching Algorithm}
\input{04.02-KM-M}

%\subsubsection{The Correctness Proof of KM-M Algorithm}
\subsection{The Correctness of KM-M Algorithm}
\input{04.03-Prove}

==> 04.01-KM.tex <==
The KM algorithm~\citep{DBLP:books/daglib/p/Kuhn10} is mainly used to solve the maximum weight maximum bipartite matching problem. By multiplying the weight of each edge in the input bipartite graph by $-1$, KM can be used to solve the minimum weight maximum bipartite matching problem in the first stage of MP$_{\text{LS}}$. Before introducing the procedure of the KM algorithm, we first introduce some definitions.

\begin{lem}
	Alternating Path. Given a bipartite graph $G = (U,V,E)$ with some edges matched. An alternating path on $G$ is a path that starts from an unmatched vertex, then traverses an unmatched edge and matched edge alternatively.
\end{lem}
	
\begin{lem}
	Augmenting Path. Given a bipartite graph $G = (U,V,E)$ with some edges matched. An augmenting path on $G$ is a special alternating path on $G$ whose starting and ending vertices are both unmatched.
\end{lem}
	
\begin{lem}
	Feasible Label. A label of a bipartite graph $G = (U,V,E)$ can be represented by assigning a value $ex_i$ on each vertex $i \in U \cup V$. A feasible label is a label that satisfies $ex_u+ex_v \ge c_{uv}$ for each edge $e_{uv} \in E$.
\end{lem}
	
\begin{lem}
	Equivalence Subgraph. An equivalence subgraph is a spanning subgraph of the original graph (a spanning subgraph contains all nodes of the original graph, but not all edges) that only contains edges satisfying $ex_u+ex_v=c_{uv}$.
\end{lem}

The procedure of the KM algorithm is shown in Algorithm \ref{alg:km}. The KM algorithm first initializes the value of each vertex. The KM algorithm sets $ex_{u} = \max_{v\in V, e_{uv}\in E}\{c_{uv}\}$ for each vertex $u \in U$, and sets $ex_v = 0$ for each vertex $v \in V$. Then KM traverses all the vertices in $U$ and tries to match each vertex $u$ by finding an augmenting path in the equivalence subgraph starting from $u$.

%The KM algorithm as follows: first set $ex_u$ of vertex in $U$ to be the maximum of the weight of the edges connected to $u$, i.e., $ex_{u\in U} = \max_{v\in V, e_{uv}\in E}\{c_{uv}\}$, and set $ex_v$ of vertex in $V$ to 0. Assume that $u_i$ denotes the $i$th element in $U$. Next, we enumerate the elements in $U$ in order from $u_1$ and try to match for $u_i$. When matching, we try to find an augmenting path in the equivalence subgraph from $u_i$.

\begin{algorithm}
	\caption{The KM algorithm}
	\label{alg:km}	
	\begin{algorithmic}[1]
		\Input $G(U,V,E)$
		\Output $\Pi$
		\Function{KM}{$G(U,V,E)$}
		\State $ex_{v \in V} \gets 0,ex_{u\in U} \gets \max_{v\in V, e_{uv}\in E}\{c_{uv}\}$, $\Pi \gets \emptyset$
		\For{$u \in U$}
		\State $\Pi \gets$ MATCH($u$, $\Pi$)
		\EndFor
		\State \Return $\Pi$
		\EndFunction
	\end{algorithmic}
\end{algorithm} 

The algorithm for matching a vertex $u \in U$ is shown in Algorithm \ref{alg:match}. The matching algorithm uses the \textit{findpath}() function (Algorithm \ref{alg:findpath}) to find an augmenting path in the equivalence subgraph from the input vertex $u$ (line 5). Once an augmenting path is found, each vertex belonging to $U$ in the augmenting path will be matched with a vertex belonging to $V$ in the augmenting path. Specifically, for an augmenting path $\{u_1,v_1,u_2,v_2,...,u_k,v_k\}$, the vertex $u_i$ is matched with the vertex $v_i$ ($i \in \{1,...,k\}$).

If the \textit{findpath}() function cannot find an augmenting path in the equivalence subgraph, then the matching algorithm tries to adjust the equivalence subgraph by adjusting the feasible label of the input bipartite graph (lines 8-18). Let $vis_x = 1$ indicates vertex $x$ is on the alternating path generated by the last search, and $vis_x = 0$ otherwise. Let $\Delta=\min_{u \in U, v \in V}\{vis_u vis_v(ex_u+ex_v-c_{uv})\}$ denotes the smallest adjustment value that makes it possible for the algorithm to find an augmenting path in the equivalence subgraph. Then the label is adjusted as follows: for each vertex $u \in U \wedge vis_u = 1$, $ex_u := ex_u-\Delta$; for each vertex $v \in V \wedge vis_v = 1$, $ex_v := ex_v+\Delta$.

Moreover, the KM algorithm designs a relaxation function $slack$ to optimize the efficiency of calculating $\Delta$ (line 8 in Algorithm \ref{alg:match}). For each vertex $v \in V$, $slack_v = \min_{u \in U, e_{uv} \in E}\{ex_u+ex_v-c_{uv}\}$ denotes the smallest value that increasing $ex_v$ by this value enables at least one edge connected with $v$ to be appeared in the equivalence subgraph. The relaxation function $slack$ is adjusted adaptively in the matching algorithm and the \textit{findpath} function. By applying the $slack$ function, the time complexity of calculating $\Delta$ can be reduced from $O(n^2)$ to $O(n)$, and the time complexity of the entire KM algorithm can be reduced from $O(n^4)$ to $O(n^3)$.

%achieved by searching the augmenting path. If not found, modifying the value of the feasible label until finding the augmenting path. 

%The modify way is as follow. Suppose $vis_x$ indicates whether $x$ is on the alternating path generated by last search, and if so, $vis_x=1$, otherwise $vis_x=0$. Let $\Delta=\min_{u \in U, v \in V}\{vis_u vis_v(ex_u+ex_v-c_{uv})\}$. Modify $ex_u=ex_u-\Delta$ for all $vis_u=1$ and $ex_v=ex_v+\Delta$ for all $vis_v=1$. 

%However, it is too slow to calculate $\Delta$ in $O(n^2)$ every time. So, introducing a relaxation function $slack$ for $v\in V$, the value of $slack_v$ is $\min_{u \in U, v \in V, e_{uv} \in E}\{ex_u+ex_v-c_{uv}\}$. Calculate the $\Delta$ by enumerating the minimum $slack_v$ of $v$ that is not in the alternating path. It reduces the time to calculate $\Delta$ to $O(n)$.

\begin{algorithm}
	\caption{The matching algorithm}
	\label{alg:match}
	\begin{algorithmic}[1]
		\Input $u\in U$, $\Pi$
		\Output $\Pi$
		\Function{match}{$u$, $\Pi$}
		\State $slack_{v\in V} \gets\infty$
		\While{$u$ is not matched}
		\State $vis_{u\in U,v\in V}\gets\text{false}$
		\If{FINDPATH($u$)}
		\State break
		\EndIf
		\State $\Delta\gets\min_{v\in V,vis_v=false}\{slack_v\}$
		\For{$u\in U, vis_u=true$}
		\State $ex_u\gets ex_u-\Delta$
		\EndFor
		\For{$v\in V$}
		\If{$vis_v = true$}
		\State $ex_v \gets ex_v + \Delta$
		\Else
		\State $slack_v \gets slack_v - \Delta$
		\EndIf
		\EndFor
		\EndWhile
		\State \Return $\Pi$
		\EndFunction
	\end{algorithmic}
\end{algorithm}

%The process of finding an augmenting path starting from a vertex $u$ is shown in Algorithm \ref{alg:findpath}. 

%The process of finding an augmenting path is as follows: enumerate all $v$ connected to $u$, and if $v$ is not matched or if an augmenting path is found for the element $u^{\prime}$ that matches $v$, then $u$ is matched with $v$ and return success. 

\begin{algorithm}
	\caption{Finding an augmenting path}
	\label{alg:findpath}
	\begin{algorithmic}[1]
		\Input $u \in U$
		\Output Whether an augmenting path is found or not
		\Function{findpath}{$u$}
		\State $vis_u\gets\text{true}$ 
		\For {$v \in V\text{ and }vis_v=\text{false}$} 
		\If{$ex_u+ex_v=c_{uv}$}
		\State $vis_v\gets\text{true}$, $u' \gets u \in U \cap e_{uv} \in \Pi$ 
		\If{$v \text{ is not matched} \vee  \text{findpath}(u')$}
		\State $\Pi \gets \Pi \backslash \{e_{u'v}\}$, $\Pi \gets \Pi \cup \{e_{uv}\}$
		\State \Return true
		\EndIf
		\Else
		\State $slack_v\gets\min\{slack_v,ex_u+ex_v-c_{uv}\}$
		\EndIf
		\EndFor
		\State \Return false
		\EndFunction
	\end{algorithmic}	
\end{algorithm} 


%This algorithm can get maximum weight matching of bipartite graph, and the minimum weight matching of bipartite graph can be got by multiplying the edge weight by -1.

==> 04.02-KM-M.tex <==
The MP$_{\text{LS}}$ algorithm performs the KM algorithm on the entire input bipartite graph in the first stage of each iteration, which is redundant. The proposed MP$_{\text{KM-M}}$ algorithm presents a simplified matching algorithm, denoted as KM-M, to calculate the minimum weight maximum matching in the first stage.
The procedure of KM-M is shown in Algorithm \ref{alg:km-m}. KM-M receives a bipartite graph $G$, a maximum matching $\Pi$ and a vertex $u \in U$ as the input, and outputs a maximum matching $\Pi$. We then explain how the KM-M algorithm works in the proposed MP$_{\text{KM-M}}$ algorithm by introducing the process of MP$_{\text{KM-M}}$ as follows.

MP$_{\text{KM-M}}$ is also an iterative heuristic algorithm and each iteration also consists of three stages like MP$_{\text{LS}}$ does. In the first stage of the first iteration of MP$_{\text{KM-M}}$, MP$_{\text{KM-M}}$ sends the original bipartite graph $G$, an empty maximum matching $\Pi = \emptyset$, and an arbitrary vertex $u \in U$ to the KM-M algorithm. Then KM-M performs the KM algorithm on $G$ and outputs a maximum matching $\Pi$ as MP$_{\text{LS}}$ does. 

The second and third stages of MP$_{\text{KM-M}}$ perform the same operations as  MP$_{\text{LS}}$ does, i.e., generates a solution to the PMMWM and improves the solution by a local search in the second stage, and adjusts the weight of an edge to $10^2c_{max}$ in the third stage. Suppose $\Pi$ is the maximum matching calculated by the first and second stages (local search in the second stage may adjust the maximum matching generated by KM-M), $e_{uv}$ ($u \in U, v \in V$) is the edge selected in the third stage, and $G'$ is the bipartite graph where the weight of edge $e_{uv}$ is just adjusted. MP$_{\text{KM-M}}$ will send $G'$, $\Pi$ and $u$ to the KM-M algorithm in the next iteration, and the KM-M algorithm only needs to remove the matching of $u$ in $\Pi$, and rematch $u$ in $G'$, which is significantly more efficient than performing KM on the entire $G'$. 

As a result, the proposed MP$_{\text{KM-M}}$ can reduce the time complexity of the first stage in each iteration except the first iteration of MP$_{\text{LS}}$ from $O(n^3)$ to $O(n^2)$. Moreover, the termination condition of MP$_{\text{KM-M}}$ is the same as that of MP$_{\text{LS}}$, i.e., MP$_{\text{KM-M}}$ stops when the solution to the PMMWM has not improved for 20 iterations.

%Since only one edge weight $e_{uv}$ is updated at each iteration, this actually only influence one vertex $u$. Therefore, we can clear the matching result of $u$, fix $c_{uv}$, and then directly use \ralg{match} to match. So that, the time complexity of each iteration except the first iteration, drop from $O(n^3)$ to $O(n^2)$.

\begin{algorithm}
	\caption{The KM-M algorithm}
	\label{alg:km-m}	
	\begin{algorithmic}[1]
		\Input $G(U,V,E)$, $\Pi$, $u$
		\Output $\Pi$
		\Function{KM-M}{$G(U,V,E)$, $\Pi$, $u$}
		\If{$\Pi \neq \emptyset$}
		\State $e_{uv} \gets$ the edge in $\Pi$ and is connected with $u$ 
		\State $\Pi \gets \Pi \backslash \{e_{uv}\}$, $\Pi \gets$ match($u$, $\Pi$)
		\Else
		\State $ex_{v \in V} \gets 0,ex_{u\in U} \gets \max_{v\in V, e_{uv}\in E}\{c_{uv}\}$, $\Pi \gets \emptyset$
		\EndIf
		\For{$u \in U$}
		\State $\Pi \gets$ match($u$, $\Pi$)
		\EndFor
		\State \Return $\Pi$
		\EndFunction
	\end{algorithmic}
\end{algorithm}

\rfig{km-m1} illustrates a maximum weight maximum matching $\Pi$ on the graph $G$ calculated by the KM algorithm. The red and black edges satisfy $ex_u+ex_v=c_{uv}$ (i.e., edges in the equivalence subgraph), and the red edges is belonging to $\Pi$. Suppose we modify the weight of the matching edge $e_{u_1 v_1}$ from $-2$ to $-10^2c_{max}$ ($-500$) and yield the new graph $G'$. The KM-M algorithm performs as follows. Firstly, as \rfig{km-m2} shows, KM-M removes the matching of $u_1$ from $\Pi$ and the modified edge $e_{u_1 v_1}$ from the equivalence subgraph. Then KM-M uses the matching algorithm (Algorithm \ref{alg:match}) to find a matching edge for $u_1$. As \rfig{km-m3} shows, the algorithm adjusts the feasible label to add edge $e_{u_1 v_2}$ into the equivalence subgraph. Finally, as shown in \rfig{km-m4}, we find an augmenting path $\{u_1,v_2,u_3,v_1\}$ (the dashed edges) and replace the edge $e_{u_3 v_2}$ with $e_{u_1 v_2},e_{u_3 v_1}$ in the matching $\Pi$. The new matching is as good as the output of the KM algorithm on the entire graph $G'$. Obviously, KM-M reduces a lot of redundant operations for calculating the matching of other edges. %, like modifying the feasible label and finding the augmenting path, by keeping the matching information. 

%\includegraphics[width=\linewidth]

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
		\setlength{\abovecaptionskip}{0.cm}
		\includegraphics[width=\linewidth]{Figure/km-m1.png}
		\caption{A matching $\Pi$ on $G$}
		\label{fig:km-m1}
    \end{subfigure}
    \hfill
   \begin{subfigure}[b]{0.24\textwidth}
        \centering
		\setlength{\abovecaptionskip}{0.cm}
		\includegraphics[width=\linewidth]{Figure/km-m2.png}
		\caption{Modify the weight of an edge}
		\label{fig:km-m2}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
		\setlength{\abovecaptionskip}{0.cm}
		\includegraphics[width=\linewidth]{Figure/km-m3.png}
		\caption{Adjust the feasible label}
		\label{fig:km-m3}
    \end{subfigure}
    \hfill
   \begin{subfigure}[b]{0.24\textwidth}
        \centering
		\setlength{\abovecaptionskip}{0.cm}
		\includegraphics[width=\linewidth]{Figure/km-m4.png}
		\caption{Find an augmenting path}
		\label{fig:km-m4}
    \end{subfigure}
\caption{An illustrate of the KM-M procedure.}
\label{fig:km-m}   
\end{figure}


%Since the improved algorithm is to reduce the matching overhead of the KM algorithm	, the improved algorithm is referred to as MP$_{\text{KM-M}}$ in this paper.

==> 04.03-Prove.tex <==
To show the correctness of KM-M, we need to briefly review the KM algorithm by the primal-dual method~\citep{DBLP:books/daglib/0069809}. The dual of the linear program of the maximum weight maximum matching problem is to minimize the sum of the feasible label.

We first present some conceptions. The primal solution is a matching $\Pi$. The dual solution is an assignment of the feasible label satisfying $ex_u+ex_v \ge c_{uv}$ for each $e_{uv} \in E$. If the primal and dual solutions obey the complementary slackness, they are optimal solutions. The complementary slackness means that each edge $e_{uv} \in \Pi$ satisfies $ex_u+ex_v = c_{uv}$, i.e., $\Pi$ is a perfect matching in the equivalence subgraph of the dual solution.

KM optimizes the dual solution until finding a perfect match in the equivalence subgraph. If a perfect matching is found, this matching is an optimal primal solution (maximum weight maximum matching) and the algorithm ends. Otherwise, there is a modification method~\citep{DBLP:journals/jacm/EdmondsK72} to decrease the sum of the feasible label and keep the dual solution feasible, which also adds new edges to the equivalence subgraph.

%We maintain a feasible dual solution. Feasibility means we ensure that $ex_u+ex_v \ge c_{uv}$ for all $e_{uv} \in E$. We try to find a primal solution that satisfies complementary slackness with respect to the current dual solution. We either find a perfect matching, or we get a vertex cover of size less than $n$. If we cannot find such solution, we find a direction of dual increase. The vertex cover in the bipartite matching instance corresponds $U^{\prime}, V^{\prime}$, a subset of the $U,V$, such that $|U^{\prime}| + |V^{\prime}| < n$ and if $ex_u+ex_v = c_{uv}$ then $u \in U^{\prime}$ or $v \in V^{\prime}$. We let $\Delta = \min_{u \in U, v \in V, e_{uv} \in E}\{ex_u+ex_v-c_{uv}\}$, and we update $u_i = u_i - \Delta$ for all $u \notin U^{\prime}$ and $v_i = v_i + \Delta$ for all $v \in V^{\prime}$. It can be proved new dual is feasible and the sum of feasible label strictly increase.

Now let's get back to the correctness of KM-M. We first present the theorem, and then the proof.

\begin{thm}
\label{thm:km-m}
Given a bipartite graph $G = (U,V,E)$ and a maximum weight maximum matching $\Pi$ calculated by the KM algorithm. If we modify the weight of exactly one edge $e_{uv} \in \Pi$ from $c_{uv}$ to a relatively large value, say $10^2c_{max}$, we only need to remove $e_{uv}$ from $\Pi$, and rematch $u$ in the new graph, to obtain the maximum weight maximum matching in the new graph.
\end{thm}

\begin{proof}

We first prove the feasibility of the dual solution. Because we only modify the weight of edge $e_{uv} \in \Pi$ from $c_{uv}$ to $10^2c_{max}$, and we known $ex_{u}+ex_{v}= -c_{uv}$, thus $ex_{u}+ex_{v} > -c^{\prime}_{u,v} = -10^2c_{max}$ holds. So the dual solution is still feasible for the current matching, indicating that the previous information can be kept. After modifying the weight of $e_{uv} \in \Pi$, only vertex $u \in U$ does not have a matching. Therefore, instead of executing the entire KM algorithm, we only need to execute \ralg{match} on $u$. 

%Because we only modify the edges in the matching, we know $ex_{u}+ex_{v}= -c_{uv}$. Obviously, $-c_{u,v} > -10^2c_{max} = -c^{\prime}_{u,v}$. So, $ex_{u}+ex_{v} \ge -c_{uv}$ holds. More precisely, satisfying $ex_{u}+ex_{v} > -c_{uv}$. So the dual solution is still feasible, which means the previous information can be kept. Before modifying this edge weight, we have a perfect matching. So now, for the vertex set $U$ only $u \in U$ does not have a matching. Instead of executing the entire KM algorithm, we only need to execute \ralg{match} on $u$. 

Then, since \ralg{match} only decreases the sum of feasible labels, we need to prove that after modifying the edge weight of $e_{uv}$, the sum of the matching weight doesn't become larger. This is easy to proof by contradiction. Assuming that the sum increases, there are two possible cases. The first one is that the modified edge is in the matching. As the edge weight decreases, the matching weight of the remaining edges increases, indicating that the previous matching is not the maximum weight maximum matching, which is a contradiction. The second one is that the modified edge is not in the matching, which can be proved in the same way. 
So \rthm{km-m} holds, and therefore KM-M is correct.

\end{proof}

==> 05-HEE.tex <==
% 这一章，描述我们改进匹配阶段启发式算法的细节。主要有三个方面，分别是更高质量的初始解生成方法，更细致的双层局部搜索策略，以及用于保证算法多样性的带精英策略的混合进化框架。
% 这一章，我们从三个方面对匹配阶段的启发式算法进行改进，在可接受的时间大幅改进解的优度。首先，采用了更高质量的初始解生成方法。对于改进解的局部搜索策略，提出了更细致的双层局部搜索。最后使用带精英策略的混合进化框架来保证算法的多样性。
In this section, we detail our improvements to the heuristic algorithm in the partition phase. The enhancements are threefold: the generation of higher-quality initial solutions, a more effective  improved local search strategy, and a hybrid evolutionary algorithm with elite strategy to ensure the diversity of the algorithm.

\subsection{Higher Quality Initial Solution For Partition}
\input{05.01-KK}

\subsection{Two-Level Improved Local Search}
\input{05.02-ILS}

\subsection{Hybrid Evolutionary Algorithm with Elite Strategy}
\input{05.03-HEE}

==> 05.01-KK.tex <==
% 对于初始解的构造，在MPLS中采用的方法是首先令所有分区为空，然后将确定匹配边的顶点按权值从大到小排序，选择当前权重和最小的分区放入。
For the construction of the initial solution, the method used in MPLS is to first make all partitions empty, and then the vertices determining the matching edges are sorted in descending order of their weights, and the partition with the current weight and the smallest is selected to be put in.
% 这个方法虽然能在多项式时间内得到一个初始解，但解的质量不够优，会影响后续启发式算法的收敛速度以及最终的优度。
While this method yields an initial solution in polynomial time, the quality of the solution is not good enough to affect the speed of convergence of the subsequent heuristic algorithms as well as their eventual superiority.

% 如果在分区中没有节点数量的限制，这个问题和k-way number partition问题是一样的，该问题的构造算法Karmarkar-Karp不是逐个节点构建单一解决方案，而是不断解决子问题并将子问题合并知道得到最终的解，能更全面的评估分区方案并作出决策。
If there is no limit on the number of vertices in the partition, this problem is the same as the multi-way number partition problem, the construction algorithm for this problem, multi-way Karmarkar-Karp, instead of constructing a single solution node by node, keeps solving subproblems and combining them to know the final solution, which can evaluate the partitioning scheme more comprehensively and make decisions.

% 接下来先描述k-way Karmarkar-Karp算法的实现细节，然后再说明如何用该算法生成partition phase的初始解
Next, we will first describe the implementation details of the multi-way Karmarkar-Karp algorithm, and then explain how to use this algorithm to generate initial solutions for the partition phase.

\subsubsection{multi-way Karmarkar-Karp algorithm}

% multi-way Karmarkar-Karp algorithm用于解决将有$n$个整数的集合$S$划分为$k$个子集，使得子集和的极差最小的问题。
The multi-way Karmarkar-Karp algorithm is used to solve the problem of partitioning a set $S$ of $n$ integers into $k$ subsets, such that the maximum difference in the sum of these subsets is minimized.
% 其用k元组的列表表示状态，每个k元组的每一维表示一个子集的和，如当k=3时，3元组$(13,12,10)$表示3个子集的和分别是13,12和10。由于该问题中我们只关心子集和之间的差值，因此可以将元组中所有数值减去该元组中的最小值，即$(13-10,12-10,10-10)=(3,2,0)$。每个元组按降序排列，元组列表按每个元组中的最大整数排序，也按降序排列。
Its state is represented by a list of k-tuples, where each element of a k-tuple corresponds to the sum of elements in a subset. For example, when $k = 3$: the 3-tuple $(13, 12, 10)$ represents that the sums of the three respective subsets are 13, 12, and 10. In addressing this problem, our focus is primarily on the differences between these subset sums. Therefore, we can adjust each tuple by subtracting its smallest value from all its elements, turning $(13, 12, 10)$ into $(13-10, 12-10, 10-10) = (3, 2, 0)$. Each tuple is organized in descending order, and the list of tuples is ordered in descending order, prioritizing the tuple with the largest integer at the forefront.

% 最初，为S中的每个整数创建一个k元组。该元组的第一个整数它的数值，其余的整数都设置为0。这些元组对应于将S的所有整数都放到第一个子集中，而其他子集中都没有整数。
Initially, a k-tuple is created for each integer in the set $S$. The first integer of this tuple is its value, and the rest of the integers are set to 0. These tuples correspond to placing all the integers of $S$ into the first subset, with no integers in the other subsets.
% 接下来进行$n-1$轮操作，每轮操作选择元组列表中前两个k元组进行合并（最大的整数最大）。为了使得合并后的k元组内整数差值尽量小，将两个k元组分别以升序和降序排列，将对应位置相加得到新的元组。如4元组$(5,3,2,0)$和$(4,4,3,0)$合并后得$(5+0,3+3,4+2,4+2)=(5,6,6,6)$。将新的k元组也只保留差值后排序，即$(5,6,6,6)=(1,1,1,0)$，最后插回到元组列表中。$n-1$轮操作后，$n$个k元组合并为1个k元组，即对应最终k个子集中整数和的相对值。
During the subsequent $n-1$ rounds, the algorithm selects and merges the first two k-tuples from the list, specifically those with the largest integers. This merging aims to minimize the disparity in integers within the resultant k-tuple. To achieve this, one k-tuple is sorted in ascending order and the other in descending order before their corresponding elements are combined to form a new tuple. For example, combining the 4-tuples $(5,3,2,0)$ and $(4,4,3,0)$ yields $(5+0, 3+3, 4+2, 4+2) = (5,6,6,6)$. This new k-tuple is then refined to emphasize the differences, transforming $(5,6,6,6)$ into $(1,1,1,0)$, which is then reintegrated into the tuple list. Following these $n-1$ rounds, the tuples coalesce into a singular k-tuple, representing the relative sums of the integers across the final $k$ subsets.
% 具体的划分子集方案可以通过合并过程得到
A specific partitioning scheme for the subsets can be derived from the merging process.

% 接下来是一个multi-way Karmarkar-Karp algorithm的完整例子。考虑初始为集合$S={26,22,19,13,8,4,3,2}$，需要将其划分为3个子集。如表格\rtbl{kk_example}所示，为multi-way Karmarkar-Karp algorithm的算法流程。
The following presents a example of the multi-way Karmarkar-Karp algorithm. Considering the initial set $S = \{26, 22, 19, 15, 8, 4, 3, 2\}$, the task is to partition it into 3 subsets. The algorithmic process is as shown in \rtbl{kk_example}.
% 初始时$i$=1，为集合中每整数生成一个3元组并将元组按最大的数进行排序。接下来每一轮，选择$T1,T2$列对应的元组进行合并，合并后重新插入元组列表，新插入的元组在下一行中加粗表示。如当$i$=2是，将元组$(26,22,0)$和$(19,0,0)$进行合并，得到$(26,22,19)=(7,3,0)$，即为$i$=3行中$T3$列的元组。当只剩一个元组时合并结束，元组$(1,0,0)$代表划分方案$\{\{26,4,3\}, \{19,13\}, \{22,8,2\}/}$，和分别为${33, 32, 32}$。
Initially, when $i = 1$, a 3-tuple is generated for each integer in the set, and these tuples are sorted by their largest number. In each subsequent round, the tuples corresponding to columns $T1$ and $T2$ are selected for merging. The merged tuple is then reinserted into the list, with its new entry in the next row highlighted in bold. For example, when $i = 2$, the tuples $(26,22,0)$ and $(19,0,0)$ are merged to form $(26,22,19) = (7,3,0)$, which is the tuple in column $T3$ for row $i = 3$. The merging process concludes when only one tuple remains. The final tuple $(1,0,0)$ represents the partition scheme $\{\{26,4,3\}, \{19,13\}, \{22,8,2\}\}$, with sums of $\{33, 32, 32\}$ respectively.

\begin{table*}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{An Example of Multi-Way Karmarkar-Karp Algorithm}
\label{tbl:kk_example}
\centering
\begin{tabular}{|c|cc|cccccc|}
\hline
i & T1 & T2 & T3 & T4 & T5 & T6 & T7 & T8 \\
\hline
1 & (26, 0, 0) & (22, 0, 0) & (19, 0, 0) & (13, 0, 0) & (8, 0, 0) & (4, 0, 0) & (3, 0, 0) & (2, 0, 0) \\
\hline
2 & \textbf{(26, 22, 0)} & (19, 0, 0) & (13, 0, 0) & (8, 0, 0) & (4, 0, 0) & (3, 0, 0) & (2, 0, 0) & - \\
\hline
3 & (13, 0, 0) & (8, 0, 0) & \textbf{(7, 3, 0)} & (4, 0, 0) & (3, 0, 0) & (2, 0, 0) & - & - \\
\hline
4 & \textbf{(13, 8, 0)} & (7, 3, 0) & (4, 0, 0) & (3, 0, 0) & (2, 0, 0) & - & - & - \\
\hline
5 & \textbf{(6, 4, 0)} & (4, 0, 0) & (3, 0, 0) & (2, 0, 0) & - & - & - & - \\
\hline
6 & (3, 0, 0) & \textbf{(2, 0, 0)} & (2, 0, 0) & - & - & - & - & - \\
\hline
7 & \textbf{(3, 2, 0)} & (2, 0, 0) & - & - & - & - & - & - \\
\hline
8 & \textbf{(1, 0, 0)} & - & - & - & - & - & - & - \\
\hline
\end{tabular}
\end{table*}

The algorithm for multi-way Karmarkar-Karp algorithm is show in \ralg{kk}

\begin{algorithm}
	\caption{The multi-way Karmarkar-Karp algorithm}
	\label{alg:kk}	
	\begin{algorithmic}[1]
		\Input $S,k$
		\Output Partition scheme
		\Function{Karmarkar-Karp}{$S,k$}
        \State $TupleList \gets$ Initial tuples of $S$
        \State $MergeInfo \gets \emptyset$  
        \While{$TupleList$'s size $>$ 2}
            \State $T1, T2 \gets$ pop the first two tuples from the $TupleList$
            \State $TNew \gets$ MergeTuple($T1$, $T2$, $MergeInfo$)
            \State Insert $TNew$ into $TupleList$
        \EndWhile
        \State $res \gets$ Obtain partition result based on $MergeInfo$
		\State \Return $res$
		\EndFunction
	\end{algorithmic}
\end{algorithm} 

%考虑节点数量限制
\subsubsection{Consider the limitation on the number of vertices}

% 通过元组的合并过程得到分区方案后，若某个分区的顶点数超过数量限制则将其随机放置在一个仍有容量的分区。后续的用启发式搜索阶段会对解进行进一步优化。
After obtaining the partitioning scheme through the tuple merging process, if the number of vertices in a partition exceeds the quantity limit, they are randomly placed in another partition that still has capacity. Subsequent heuristic search stages will further optimize the solution.


==> 05.02-ILS.tex <==
% 局部搜索的目标是通过改变某些顶点的partition继续优化目标。令partition的权重为其中包含的顶点的权重和, partition阶段的目标是最小化partition权重的最大值，因此局部搜索主要通过将当前权重最大的partition中的顶点与其他partition进行交换来优化目标。
The goal of the local search is to further optimize the solution by altering the partition of certain vertices. Define the weight of a partition as the sum of the weights of the vertices it contains. 

The objective of the partition phase is to minimize the maximum weight of any partition. Consequently, the local search primarily focuses on optimizing this objective by exchanging vertices from the partition with the current highest weight with those from other partitions. This approach aims to balance the partition weights more effectively.

% 我们提出的Improved local search是一个二级的局部搜索。将局部搜索策略分为两种，首先一级局部搜索尝试将权值最大的partition和最小的partition中的顶点进行交换，使得权值和尽量平均。若该策略无法继续对目标进行优化，则使用二级局部搜索尝试将权值最大的partition和其余所有partition都进行交换。
% 这两级局部搜索尝试的交换操作也有所区别，分别注重搜索的深度和广度，后续会分别详细描述。
We propose an Improved Local Search, a two-level local search strategy. The local search strategy is divided into two levels. Initially, the first-level local search attempts to exchange vertices between the partition with the highest weight and the one with the lowest, aiming to achieve a more balanced distribution of weight sums. If this strategy no longer yields further optimization of the objective, the second-level local search is employed. This level involves attempting exchanges between the partition with the highest weight and all other partitions, thereby exploring a broader range of potential improvements.
The swap operations attempted in these two levels of local search are distinct, with each level emphasizing either the depth or breadth of the search. These differences in approach will be detailed in subsequent sections

The procedure of improved local search is show in \ralg{ILS}.

\begin{algorithm}
	\caption{Improved Local Search}
	\label{alg:ILS}	
	\begin{algorithmic}[1]
		\Input $Sol$
		\Output $Sol$
		\Function{ImprovedLocalSearch}{$S,k$}
        \State $isUpdate \gets true$
        \While{$isUpdate$}
            \State $isUpdate, Sol \gets$ LocalSearchMaxMin($Sol$)
            \If{$isUpdate = false$}
                \State $isUpdate, Sol \gets$ LocalSearchMaxAll($Sol$)
            \EndIf
        \EndWhile
		\State \Return $Sol$
		\EndFunction
	\end{algorithmic}
\end{algorithm} 

% 
\subsubsection{The first-level local search}

% 选择权重最大和最小的两个分区$P_{max}$，$P_{min}$中的顶点进行交换。首先将$P_{min}$中的顶点按权重进行排序。尝试将$P_{max}$中的一个顶点与$P_{min}$中若干连续的顶点进行交换。选择令两个partition差值最小的操作执行。
Select vertices from the two partitions with the largest and smallest weights, $P_{max}$ and $P_{min}$, respectively, for exchange. First, sort the vertices in $P_{min}$ by their weights. Attempt to swap a vertex from $P_{max}$ with several consecutive vertices in $P_{min}$. Execute the operation that minimizes the difference between the two partitions.

% 这级的搜索由于只考虑两个partition，着重考虑搜索的深度。会尝试大量的交换方案，并选择最优的执行。在改进解的同时使得分区方案更均衡。在代码实现中也根据单调性见少$P_min$中顶点的枚举范围，提高效率
This level of search, focusing solely on two partitions, will explore a vast array of swap scenarios, selecting the most optimal one for execution. This not only improves the solution but also leads to a more balanced partitioning scheme. In the code implementation, the enumeration range of vertices in $P_{min}$ is also reduced based on monotonicity, thereby enhancing efficiency.

\subsubsection{The second-level local search}

% 选择权重最大分区$P_{max}$和其他所有分区中的节点进行交换。尝试将一个$P_{max}$中的顶点和一个其他分区的一个顶点进行交换。将分区按权值从小到大遍历，执行第一个找到的能优化目标函数的操作。
Select vertices from the partition with the highest weight, $P_{max}$, for exchange with vertices from all other partitions. Attempt to swap a vertex from $P_{max}$ with a vertex from another partition. Traverse the partitions in ascending order of their weights and execute the first operation found that can optimize the objective function.

% 这级的搜索策略考虑所有partition，着重搜索的宽度。找到可行动作直接执行，在优化目标函数的同时改变$P_{max}$中的顶点构成。从而，下一轮的一级搜索可能有交换操作继续优化目标函数。
This level of the search strategy takes into account all partitions, emphasizing the breadth of the search. Upon finding a feasible action, it is executed immediately, optimizing the objective function while simultaneously changing the composition of vertices in $P_{max}$. As a result, the next round of first-level search may involve swap operations that continue to optimize the objective function.

% 若仍没有可以改进目标函数的操作则会尝试使用2-way Karmarkar-Karp算法对$P_{max}$和$P_{min}$中的节点进行重新分配。
If there are still no operations that can improve the objective function, the strategy will consider employing the 2-way Karmarkar-Karp algorithm to redistribute the vertices within $P_{max}$ and $P_{min}$.

==> 05.03-HEE.tex <==
% Hybrid evolutionary算法参考种群的思想，同时维护问题的多个解，并通过杂交算子在原有解的基础上产生新的解，从而保证算法的疏散性。
The hybrid evolution algorithm draws inspiration from the concept of a population, maintaining multiple solutions to a problem simultaneously. It generates new solutions based on existing ones through crossover operator. This approach ensuring the diversity of the algorithm, helping to escape from local optima and potentially leading to more globally optimal solutions.
% thereby ensuring the diversity of the algorithm.

% 对于上一节的Improve local search算法每次都在当前解的基础上进行修改来提升解的质量，容易陷入局部最优解。因此，我们使用Hybrid evolutionary的方式来增加算法的疏散性
The Improved Local Search algorithm, as discussed in the previous section, modifies the current solution to enhance its quality, which can easily lead to local optima. Therefore, We employ a hybrid evolutionary algorithm with elite strategy(HEE) to increase the diversity of the search while simultaneously ensuring operational efficiency.
% 接下来分别算法的设计细节

The procedure of HEE is show in \ralg{HEE}.
% 算法首先初始化种群$pops$（第2行），并通过improved local searc优化初始种群中的解（第3行到第5行）。然后通过种群的演化搜索更多的解（第6行到第23行）。具体的，每次迭代分别选择种群中的精英解$sol_{elite}$和随机解$sol_{random}$（第6行到第23行为）。将这两个解通过交叉算子生成新的解$sol_{new}$（第10行），并使用improved local search进行优化（第11行）。若$sol_{new}$优于$sol_{elite}$，则在$pops$进行替换（第29到第31）。若其优度与$sol_{random}$或$sol_{elite}$相同，则认为解$sol_{random}$难以为精英解带来多样性，将其从$pops$中移除（第33到34行）。否则，$sol_{new}$仍有继续保留在pops$中增加多样性的价值，将其替换$pops$中的$sol_{random}$（第36到37行）。
The algorithm firstly initializes the population $pops$ (line 2) and optimizes the solutions in the initial population through improved local search (lines 3 to 5). It then searches for more solutions through the evolution of the population (lines 6 to 23). Specifically, in each iteration, it selects an elite solution $sol_{elite}$ and a random solution $sol_{random}$ from the population (lines 8 to 9). These two solutions are combined using a crossover operator to generate a new solution $sol_{new}$ (line 10), which is then optimized using improved local search (line 11). If $sol_{new}$ is better than $sol_{elite}$, it replaces the latter in $pops$ (lines 29 to 31). If its quality is the same as that of $sol_{random}$ or $sol_{elite}$, it is considered that $sol_{random}$ is unlikely to bring diversity to the elite solutions, and is therefore removed from $pops$ (lines 33 to 34). Otherwise, $sol_{new}$ still has value in adding diversity to $pops$, and it replaces $sol_{random}$ in the population (lines 36 to 37).

\begin{algorithm}
	\caption{Hybrid Evolutionary Algorithm with Elite Strategy}
	\label{alg:HEE}	
	\begin{algorithmic}[1]
		\Input $w,k$
		\Output Partition scheme
		\Function{HEE}{$S,k$}
        \State Initial $pops$
        \For{$sol \in pops$}
            \State $sol \gets$ ImproveLocalSearch($sol_{new}$)
        \EndFor
        \State $noImproTurn \gets 0$  
        \While{$|pops| > 1$ and $noImproTurn \leq LIMIT$}
            \State $sol_{elite} \gets$ best solution of $pops$
            \State $sol_{random} \gets $ random select solution from population
            \State $sol_{new} \gets$ CrossOver($sol_{elite}$, $sol_{random}$)
            \State $sol_{new} \gets$ ImproveLocalSearch($sol_{new}$)
            \If {$sol_{new}$ better than $sol_{elite}$}
                \State $noImproTurn \gets 0$
                \State $pops \gets pops \backslash sol_{elite}, pops \gets pops \cup sol_{new}$ 
            \Else
                \If {$sol_{new}$ value same as $sol_{elite}$ or $sol_{random}$}
                    \State $pops \gets pops \backslash sol_{random}$
                \Else
                    \State $pops \gets pops \backslash sol_{random}, pops \gets pops \cup sol_{new}$ 
                \EndIf
                \State $noImproTurn \gets noImproTurn + 1$
            \EndIf
        \EndWhile
		\State \Return best solution of $sols$
		\EndFunction
	\end{algorithmic}
\end{algorithm} 

Following is a detailed description of the design aspects of this algorithm.

\subsubsection{Initial Population}

% 种群的初始解需要保证多样性，因此采用多种方式生成初始解：（1）multi-way Karmarkar-Karp算法（2）采用贪心算法，将顶点权重按从大到小依次放入分区。每次选择当前权重最小的分区放置（3）在贪心算法的基础上加入随机性，当顶点选择放入的partition时，有一定概率不选择当前权重最小的分区，而是随机选择一个容量为到达上限的分区。这个概率设为50%。
To ensure diversity in the initial solutions of the population, we employ various methods to generate these initial solutions:(1) multi-way Karmarkar-Karp algorithm (2) greedy algorithm: vertex weights are sorted in descending order, and each vertex is sequentially placed into a partition. The vertex is always placed in the partition with the current smallest weight sum to maintain balance. (3) random algorithm: this approach adds an element of randomness to the greedy algorithm. When assigning a vertex, rather than always opting for the partition with the smallest weight sum, there's a 50\% chance of randomly selecting a partition that still has available capacity.

% 通过方法一和方法二各生成一个解，其余解通过方法三生成。在保证种群优度的同时，通过方法三引入解的不同特征，满足多样性的需求。
One solution is generated using Method 1 and another using Method 2, while the remaining solutions are generated through Method 3. This approach ensures the quality of the population while introducing diverse characteristics into the solutions via Method 3, thereby fulfilling the requirement for diversity.
% 经过测试，在算法中，令种群的大小为5。能够同时保证效率和优度。
After testing, it has been determined that setting the population size to 5 in the algorithm effectively balances efficiency and solution quality.

\subsubsection{Crossover Operator}

% 交叉算子用于模拟生物遗传中的交叉过程，根据两个父代解生成新的个体。结合两个父代解中的特征，创造新的特征组合并引入一定的随机性，保证算法的多样性。
The crossover operator is used to simulate the crossing-over process in biological genetics, creating new individuals based on two parent solutions. By combining features from both parents, it creates new feature combinations and introduces a degree of randomness. This ensures diversity in the algorithm, mirroring the genetic diversity seen in natural selection and evolution.

% 我们采用了解决图着色问题中用到的Greedy Partition Crossover(GPX)方法，在两个父代中交替的选择当前含有节点数量最多的Partition，若有多个则随机选择一个，加入到子代的解中。已经加入自带的顶点后续不再考虑，可以视为在父代中删除。直到进行$k$轮后，可能仍有一些节点未加入子代的解中，则随机的加入未到达容量限制的partition。
We have adopted the Greedy Partition Crossover (GPX) method, commonly used in solving graph coloring problems. In this method, we alternately select the partition with the most vertices from each of the two parent solutions. If there are multiple such partitions, one is chosen randomly to be included in the child's solution. Vertices that have been added are not considered in subsequent steps, effectively treating them as removed from the parents. After $k$ rounds of this process, there may still be some vertices not included in the child's solution. These remaining vertices are then randomly added to any partition that has not yet reached its capacity limit. 

% 用不用加一个图？

\subsubsection{Elite Strategy}

% 一般的hybrid evolution算法每次随机挑选两个种群中的解作为父代进行杂交。这样虽然能保证算法的多样性，但效率不够高。我们的方法对父代的选择进行改进，每次都将种群中最优的个体作为其中一个父代，另一个父代仍采用随机的方式。我们称这种策略为精英策略，最优的个体为精英解$sol_{elite}$。令随机生成的父代以及产生的子代分别为$sol_{random}$和$sol_{new}$
In typical hybrid evolutionary algorithms, two solutions from the population are randomly selected as parents for crossover. While this approach ensures diversity in the algorithm, it is not particularly efficient. Our method improves upon the selection of parents by consistently choosing the best individual in the population as one of the parents, while the other parent is still selected randomly. We refer to this approach as the elite strategy, with the best individual being termed the elite solution. 

% 换种方式取理解，每次杂交都是通过在精英解中加入种群中其他解的特征，尝试对精英解继续改进。使得每轮迭代更有目的性，在大幅提升效率的同时也保证了一定的多样性。 
Each crossover event in our approach involves incorporating features from other solutions in the population into the elite solution, with the aim of further improving the elite solution. This method ensures that each iteration is more targeted, significantly enhancing efficiency while also maintaining a degree of diversity. By focusing on refining the elite solution with attributes from various other solutions, we strike a balance between intensifying the search around the most promising areas and exploring new possibilities, thereby optimizing the algorithm's performance.

% 为了配合精英策略，子代更新种群的策略也和常规的方法有区别。在对子代进行改进后，若当生成子代优于精英解时，该子代成为新的精英个体，替换掉种群中原先的精英解。若子代的目标函数值等于其中一个父代，我们认为$sol_{new}$和$sol_{random}$没有合适的特征来改进精英解，并且多样性也不够。所以不将$sol_{new}$加入种群，并且将$sol_{random}$从种群中移除，来加速迭代过程。
To complement the elite strategy, the approach for updating the population with child also differs from conventional methods. After optimal the child, if it proves superior to the elite, this child becomes the new elite individual, replacing the previous elite in the population. If the child's objective function value is equal to one of its parents, we infer that neither $sol_{new}$ nor $sol_{random}$ possess suitable characteristics to improve upon the elite, and their diversity is also insufficient. Therefore, $sol_{new}$ is not added to the population, and $sol_{random}$ is removed to accelerate the iteration process. This strategy streamlines the search process by focusing on the most promising solutions.

% 算法的结束条件为，种群中只剩下一个解或者在一定轮数的迭代内没有对精英解进行改进。经过测试，在算法中，这个轮数设为种群数量的4倍。
The termination condition for the algorithm is set to occur when only one solution remains in the population or if there is no improvement in the elite solution over a certain number of iterations. Through testing, this number of iterations has been determined to be four times the size of the population.









==> 06-Exp.tex <==
% 这一章首先介绍新数据集得生成方式，然后用该数据集对本文提出得算法进行测试。
This section first introduces the method for generating new datasets, and then utilizes these datasets to test the algorithm proposed in this paper.

\subsection{New Instance Set}
\input{06.01-DS}

\subsection{Result}
\input{06.02-Exp}

==> 11-Intro.tex <==
\IEEEPARstart{I}{n} this paper, we consider a typical NP-hard problem, the Partitioning Min-Max Weighted Matching (PMMWM) problem \cite{a1}. 
% The PMMWM is defined by a weighted bipartite graph $G(U,V,E)$ with disjoint vertex sets $U$, $V$ and edge set $E = \{e_{uv}|u \in U, v \in V\}$, where $U$ needs to be partitioned into $m$ disjoint partitions with no more than $\bar{u}$ vertices each.
The PMMWM is defined by a weighted bipartite graph $G(U, V, E)$ with disjoint vertex sets $U$, $V$ and edge set $E = \{e_{uv} | u \in U, v \in V\}$, where the weight of each edge $e_{uv}$ is denoted by $w(e_{uv})$. Set $U$ needs to be partitioned into $m$ disjoint partitions with no more than $\bar{u}$ vertices each.
Given a maximum matching on $G$, the weight of a partition is defined as the sum of the edge weights for the edges matching the vertices in the partition. The goal of the problem is to find a matching and a partition to minimize the largest weight of the partitions. The PMMWM is an NP-hard problem in the strong sense \cite{a1}.

\begin{figure}[t]
\centering
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{Figure/example.png}
  \caption{A feasible solution}
  \label{fig:example1}
\end{subfigure}\hfil
\begin{subfigure}{0.24\textwidth}
  \includegraphics[width=\linewidth]{Figure/example-better.png}
  \caption{An improved solution}
  \label{fig:example2}
\end{subfigure}
\caption{A PMMWM solution example.}
\label{fig:pmmwm}
\end{figure}

\rfig{example1} illustrates a feasible solution to a PMMWM instance. The colored edges indicate the maximum matching edges and the associated weights are marked beside. The left part of the bipartite graph, $U=\{u_1,u_2,...,u_6\}$, is divided into three partitions, $U_1$, $U_2$ and $U_3$ labeled with different colors. The weights of the three partitions are 4, 2 and 5. The value of the objective function is 5. 

We consider two different ways to optimize the objective function.
The first is to modify the partition strategy. We can move $u_6$ to $U_2$, then the weights of the three partitions become 4, 3, and 4. The objective function value is 4. 
The second is to modify the matching strategy. For $u_3,u_5$, if we replace the current matching edges $e_{u_3 v_6}, e_{u_5 v_2}$ with edges $e_{u_3 v_2},e_{u_5 v_6}$, then the weights of the partitions become 4, 4, 4, as shown in \rfig{example2}. Although the total weight of the matching edges is increased, the final objective function is reduced to 4.

\citet{a1} show an application of the PMMWM at small to medium sized seaports. The seaports include long-term storage areas and temporary storage areas. The vertex set $U$ denotes the empty slots in the long-term storage area, the vertex set $V$ denotes the containers in the temporary storage area, and the edge weight $w(e_{uv})$ for an edge $e_{uv} \in E$ denotes the cost required to move the container $v$ to the empty slot $u$. 
The parameter $m$ indicates the number of available telescopic stackers and $\bar{u}$ indicates the upper limit of the number of containers that can be handled by one telescopic stacker. Suppose the cost of a telescopic stacker equals to the total cost of moving its containers, the goal of the problem is to minimize the maximum cost among the telescopic stackers.
%the cost of the telescopic stacker with the maximum cost.

We find another application of the PMMWM that is related to the task allocation. Suppose there are $n$ workers, $n$ tasks, and $m$ machines in a workshop. Each task should be performed on a machine by a worker, each worker performs only one task, and each machine can take at most one task at a time. The vertex set $U$ denotes the workers, $V$ denotes the tasks, and the edge weight $c_{uv}$ denotes the spending time of performing task $v$ by worker $u$. The parameter $\bar{u}$ indicates the maximum number of tasks that can be performed by each machine per day (working period). The goal of the problem is to determine the matching between workers and tasks, and the partition of workers to machines, so as to minimize the longest spending time among the machines. % of the machine with the longest spending time.

The PMMWM is an extension problem of the Min-Max Weighted Matching (MMWM) problem \citep{a2}. MMWM is motivated by the container transshipment in a rail-road terminal. MMWM has the same objective function as PMMWM, but the partitioning of the vertices is given. So, MMWM only needs to decide the matching result. \citet{a2} prove that the MMWM is NP-hard in the strong sense and develop heuristics to find the matching that the average gap to the optimal solution is less than 1\%. However, in some practical applications, the partition also needs to be determined. So, \citet{a1} propose the PMMWM problem.

% When there is only one partition (i.e., $m = 1$), the PMMWM can be reduced to an assignment problem that just needs to find a maximum matching with minimum weight. For the assignment problem, \citet{a3} propose an exact polynomial-time algorithm called the Hungarian method which is also denoted as the KM algorithm. 
% Moreover, the KM algorithm inspired \citet{primal-dual} to propose the primal-dual method for linear programming, which is widely used for various combinatorial optimization problems. In this paper, we also use the primal-dual method to prove the correctness of the proposed KM-M algorithm. 

The PMMWM problem can be decomposed into two stages, match and partition, and can be solved either exactly or heuristically. 
The match stage requires solving the minimum weight perfect matching problem, which can be transformed into the classic Maximum-Weight Perfect Matching (MWPM) problem \cite{MWPM, AP} by inverting the weight values. The exact polynomial-time algorithm, KM algorithm \cite{KM} (also called Hungarian method), can find the optimal solution of the MWPM problem.          
% The partition stage需要把顶点分配到有容量上限的分区，最小化节点权重和最大的分区。这个问题在不同的应用场景被提出并解决，如Multiprocessor Scheduling Problem和multi way pratition problem.
The partition stage requires distributing vertices into partitions with a capacity limit, aiming to minimize the weight sum of the maximum partition. This problem has been addressed in various application scenarios, such as the Multiprocessor Scheduling problem \cite{RP} and the Parallel Machine Scheduling problem \cite{PMS}. Multi-way Number Partition (MNP) problem \cite{NPAll-1,NPAll-2,NPAll-3} is another similar problem aiming to minimize the difference in the weight sum across partition. 
% 解决该类问题的方法大致有两类：optimal algorithm, approximate algorithm and heuristic algorithm. 最优算法如SNP,MOF,BSBCP,CIW虽然能得到最优解，但只能应用在n较小的情况，在n=60下就需要花费1分钟左右的运行时间。approximate algorithm,如GA和KK能较快的得到一组保证质量的解，但往往离最优解有一定距离。Heuristic algorithm介于这两者之间，如DIMM-SS,ICSA能在一定时间内得到不错的解。
Algorithms for solving these problem generally fall into three categories: optimal algorithms, approximate algorithms, and heuristic algorithms. Optimal algorithms like SNP \cite{SNP}, MOF \cite{MOF}, BSBCP \cite{BSBCP} , and CIW \cite{CIW}, although capable of obtaining optimal solutions, are only applicable to small instance. Approximate algorithms, such as GA \cite{GA1} and KK \cite{KK}, can quickly produce a quality-guaranteed solution, but often have a large gap from the optimal solution. Heuristic algorithms fall between these two, such as DIMM \cite{DIMM} and ICSA \cite{ICSA},  can achieve satisfactory solutions within a certain time. 
% PMMWM问题的算例超过了精确算法能解决的规模，而近似算法的优度又不够，因此一般采用启发式算法求解partition stage。
The scale of the PMMWM problem instances exceeds the capacity of exact algorithms, and the quality of solutions provided by approximate algorithms is not sufficient. Therefore, heuristic algorithms are generally used to solve the partition stage.

 \citet{a1} proposed the MP$_{\text{LS}}$ algorithm by applying the KM algorithm and a local search respectively to these two stages, and conducting iterative optimization.
\citet{7376822} employs integrated approaches to directly solve the PMMWM problem. They propose a heuristic based on tabu search \citep{DBLP:journals/informs/Glover89,DBLP:journals/informs/Glover90} and a genetic algorithm~\citep{DBLP:books/daglib/0019083}. But these two algorithms are not as effective as the MP$_{\text{LS}}$ algorithm. Therefore, MP$_{\text{LS}}$ is still the state-of-the-art algorithm for the PMMWM.

% However, in some practical applications, the partition also needs to be determined. So, \citet{a1} propose the PMMWM and decompose the problem into two stages, matching and partitioning, and solve them either exactly or heuristically. They propose two different heuristic frameworks with different order of the matching and partitioning phases. For the Partition-Match framework, they propose two heuristics called PM$_{\text{BPS}}$ and PM$_{\text{REG}}$. For the Match-Partition framework, they propose other two heuristics called MP and MP$_{\text{LS}}$. By performing extensive experiments, \citet{a1} conclude that the MP$_{\text{LS}}$ algorithm is the best-performing one among the four algorithms, and is also robust against changes in the graph structure.
% \citet{7376822} also apply PMMWM to the intermodal transport, and propose a heuristic based on tabu search \citep{DBLP:journals/informs/Glover89,DBLP:journals/informs/Glover90} and a genetic algorithm~\citep{DBLP:books/daglib/0019083}. They propose three neighborhood structures for the tabu search heuristic and a crossover operator for the genetic algorithm. But these two algorithms are not as effective as the MP$_{\text{LS}}$ algorithm. Therefore, MP$_{\text{LS}}$ is still the best-performing algorithm for the PMMWM. 
% In this work, we select MP$_{\text{LS}}$ as the baseline algorithm, and our proposed MP$_{\text{KM-M}}$ algorithm significantly outperforms MP$_{\text{LS}}$ on the algorithm efficiency while keeping the same effectiveness.


% In this work, we proposed FMP\_HEE algorithm significantly outperforms MP$_{\text{LS}}$ both on efficiency and optimality.

% In this work, 我们提出了FMP_{HEE}算法。在整体设计上采用matchinng-partition框架。

% 在这篇文章中，我们仍然采用分离式的框架，即Match-Partition框架，提出Fast Iterative Match-Partition Genetic Algorithm with Elite Strategy来解决PMMWM问题.
% 我们认为the decomposition approaches相较于integrated approaches能更高效的探索解空间，因此在这篇文章中，我们采用Match-Partition框架，提出了Fast Iterative Match-Partition Genetic Algorithm with Elite Strategy来解决PMMWM问题

Based on previous experimental \cite{7376822}, the decomposition approaches can explore the solution space more efficiently than the integrated approaches. Therefore, in this article, we adopt the Match-Partition framework and propose the Fast Iterative Match-Partition Genetic Algorithm with Elite Strategy(FIMP-GAE) to solve the PMMWM problem.

FIMP-GAE is an iterative heuristic algorithm, and each iteration consists of three stages. 
%The first stage generates a maximum matching $\Pi$ of $G = (U,V,E)$, and the second stage calculates a partition $\mathcal{P}$ of $U$ that satisfies constraints of the problem. Then the combination of $\mathcal{P}$ and $\Pi$ results is a feasible solution. In the third stage, FIMP-GAE makes a slight adjustment on the weight matrix of $E$ and then returns to the first stage of the next iteration, which can help the algorithm to explore a broader solution space. We denote $G'$ to be the bipartite graph where the edge weight matrix is adjusted. Starting from $G' = G$, the FIMP-GAE algorithm repeats the three stages until a termination condition is met. Implementation details of the three stages are as follows.
% 在第一阶段，即match stage，我们需要解决MSWM problem. 
In the first phase(match stage), we use exact algorithm to solve the MWPM problem. Although the KM algorithm can find the optimal solution, its running efficiency is not satisfying.
% 由于每轮迭代中只对图作细微的调整，从第二轮迭代开始可以复用之前大量的匹配信息，从而减少冗余操作。
Since only minor adjustments are made to the graph in each iteration, a large amount of matching information from previous iterations can be reused to reduce redundant operations. Guided by this analyse, we proposed the KM-M algorithm, which accelerates the theoretical complexity of the match stage from $O(n^3)$ to $O(n^2)$ while ensuring the optimality of the matching.
% 演化算法相较于用于MP_LS中的局部搜索能提供更好的全局搜索能力，并且提供更好的鲁棒性和灵活性.genetic algorithm 作为演化算法的一种，通过
Then, we propose a genetic algorithm with elite strategy (GAE) for the second stage (partition stage). The genetic algorithm (GA) \cite{Genetic1,Genetic2,Genetic3}, as a type of evolutionary algorithms \cite{Evolution1,Evolution12,Evolution13}, compared to the local search (used in MP$_{\text{LS}}$), provide better global search capabilities, along with enhanced robustness and flexibility. GAE use approximate algorithms, Greedy algorithm \cite{GA1} and multi-way Karmarkar-Karp algorithm (KK) \cite{KK}, to generate initial population, and generate new populations by proposed Greedy Partition Crossover. Each solution obtained through initialization and crossover is optimized by a proposed Multi-Level Local Search (MLLS) algorithm. To accelerate the evolution of the population, we introduce the Elite Strategy \cite{GeneticElite1,GeneticElite2,GeneticElite3}. This means that in each crossover, the optimal individual is always be selected. 
%In the second stage(partition stage), we proposed HEE algorithm to calculates a partition scheme $\mathcal{P}$. In this stage, the maximum matching $\Pi$ of $G'$ is fixed, then the problem can be regarded as a restricted partitioning problem of $U$, by setting the weight of each vertex $u \in U$ to $w(u) = w(e_{uv}), e_{uv} \in \Pi$ (note that when calculating the partition in this stage, $w(e_{uv})$ is always the original weight of edge $e_{uv}$). HEE use a hybrid evolution strategy and corresponding crossover operators to ensure the diversity of the algorithm. Initially, we use multi-way Karmarkar-Karp algorithm~\cite{KK} and greedy strategy to generate initial population.
%Each solution obtained through initialization and crossover is optimized by a proposed three-level local search algorithm. To accelerate the evolution of the population, we introduce the elite strategy~\cite{GeneticElite1,GeneticElite2,GeneticElite3}. This means that in each crossover, the optimal individual is always one of the parents.
Finally, in the third stage, FIMP-GAE bans an edge in $G'$ for a certain number of iterations to adjust the bipartite matching solution in the next iteration, which can help the algorithm to explore a broader solution space.
%Let $k = \mathop{\arg\max_{k \in \{1,...,m\}}{\{\sum_{u \in U_k, e_{uv} \in \Pi}{w(e_{uv})}\}}}$, then the selected edge $e \in \Pi$ is an edge with the maximum weight among the current edges of $\Pi$ that are incident to vertices of component $U_k$. The FMP\_HEE algorithm 
% ban the edge $e$ for a certain number of iterations, consequently modifying the matching scheme for the subsequent iteration. 
% changes the weight of $e$ in $G'$ to a large value ($10^2 c_{\max}$ in default, where $c_{\max}$ is the maximum edge weight in the input graph) to largely reduce the probability that this edge will belong to the matching calculated in the first stage of the next iteration. 
% 但是如果这轮迭代得到的解和最优解的差距到达一定值时，将会把当前所有禁用的边以一定概率马上解禁。当边解禁的同时也需要用KM-M算法对相关节点重新规划匹配方案。
However, if the difference between the solution obtained in the current iteration and the optimal solution reaches a certain threshold, all currently banned edges will be unbanned with a certain probability, we refer to it as the Edge Recovery Strategy. When an edge is unbanned, it is also necessary to use the KM-M algorithm to re-plan the matching scheme for the related vertices.

% The MP$_{\text{LS}}$ algorithm stops when the solution to the PMMWM has not improved for 20 iterations.

\begin{comment}
% 我们总结了MPLS算法的两个缺点，并针对这两个方面提出改进方案：（1）matching阶段效率较低（2）partition阶段优度较低
In this work, we analyze the MP$_{\text{LS}}$ algorithm proposed by \cite{a1}. It solves this problem by Matching-Partition(MP) framework, which employs the KM algorithm for matching phase and applies a local search strategy for partition phase. As follows, we find two main weakness of the MP$_{\text{LS}}$ algorithm and propose improvement strategies for these two aspects:

(1) MP$_{\text{LS}}$ is an iterative algorithm, and at each iteration it adjusts the edge weight matrix of the bipartite graph to generate a different initial maximum matching by an exact algorithm. In the matching phase,MP$_{\text{LS}}$ applies a complete matching algorithm to the bipartite graph each iteration, which becomes a time bottleneck. However,  the modified bipartite graph does not change much at each iteration, there are many redundant operations that can be optimized. 
% 因此，我们提出了KM-M算法替换MP框架中每轮匹配使用的KM算法，得到更高效的框架FMP
Hence, we propose the KM-M algorithm to replace the KM algorithm used in each round of matching within the MP framework, resulting the efficent Fast Matching-Parition(FMP) framework, which reuses the matching results of the edges that their weights are not changed in the last iteration, and hence reduces the time complexity from $O(n^3)$ to $O(n^2)$ of the matching phase while maintaining the resulting quality.

(2) In the partition phase, the initial solution algorithm of MP$_{\text{LS}}$ primarily emphasizes efficiency, but there is still considerable room for improvement in the quality of the solution. The subsequent local search algorithm only considers simple exchange actions and neglects diversity, making it susceptible to falling into local optima and directly affecting the quality of the solution. In this paper, we  employs the multi-way Karmarkar-Karp algorithm for the K-way number partition problem to generate higher-quality initial solutions. Following this, we proposed a efficient two-level local search strategy to enhance the quality of the solution called Improved Local Search(ILS). Initially, It attempts to enhance the solution's quality through a certain extent of search(first level). If these actions fail to yield improvements, the strategy then shifts to a more fine-grained search approach(second level). 
Furthermore, we propose a hybrid evolution strategy and corresponding crossover operators to ensure the diversity of the algorithm. Each solution obtained through crossover is optimized by the ILS algorithm. To accelerate the evolution of the population, we propose the concept of elite individuals.
\end{comment}

% 另外，对数据集分析后，我们按二分图的疏散性和密度对数据进行分类。按这种方式对之前提出的数据集进行整理以及补充，使得能对算法进行更全面的实验及分析。
Furthermore, we classify the instances based on the consistency and density of the bipartite graph and generate new benchmarks compatible with previous studies. We conduct extensive experiments with the FIMP-GAE and analyze the characteristics of the PMMWM problem based on these new benchmarks.

The remainder of the paper is organized as follows.
\rsec{prob} introduces a detailed formulation of the PMMWM problem. Subsequently, \rsec{p} presents the preliminaries, including the KM algorithm and the multi-way Karmarkar-Karp algorithm. \rsec{alg} presents the details of the FIMP-GAE algorithm. The process of dataset generation and the corresponding test results are detailed in \rsec{exp}. Finally, \rsec{con} summarizes the main conclusions of this paper.
% 第四章详细描述了KMP框架以及证明其正确性，第五章详细描述了匹配阶段使用的技巧。第六章描述了数据集的生成方式以及测试结果
 % We describe the related works in Section 2, and formulate the PMMWM problem in Section 3. Section 4 briefly introduces the MP$_{\text{LS}}$ algorithm, and Section 5 details the proposed MP$_{\text{KM-M}}$ algorithm and proves the correctness. Section 6 reports the results of the experiment, and Section 7  summarizes the main conclusion of this paper.



==> 13.01-RS.tex <==
The PMMWM is an extension problem of the Min-Max Weighted Matching (MMWM) problem \citep{a2}. MMWM is motivated by container transshipment in a railroad terminal. MMWM has the same objective function as PMMWM, but the partitioning of the vertices is given. So, MMWM only needs to decide the matching result. \citet{a2} prove that the MMWM is NP-hard in the strong sense and develop heuristics to find the matching that the average gap to the optimal solution is less than 1\%. %one percentage. 

When there is only one partition (i.e., $m = 1$), the PMMWM can be reduced to an assignment problem that just needs to find a maximum matching with minimum weight. For the assignment problem, \citet{a3} propose an exact polynomial-time algorithm called the Hungarian method, which is also denoted as the KM algorithm. The KM algorithm is applied on the matching process of MP$_{\text{LS}}$~\cite{a1}. Moreover, the KM algorithm inspired \citet{primal-dual} to propose the primal-dual method for linear programming, which is widely used for various combinatorial optimization problems. In this paper, we also use the primal-dual method to prove the correctness of the proposed KM-M algorithm. 

However, in some practical applications, the partition also needs to be determined, for instance, in small to medium-sized seaports where containers are handled by reach stackers. So, \citet{a1} propose the PMMWM and decompose the problem into two stages, match and partition, and solve them either exactly or heuristically. They propose two different heuristic frameworks with different orders of the matching and partitioning phases. For the partitioning-matching framework, they propose two heuristics called PM$_{\text{BPS}}$ and PM$_{\text{REG}}$. For the matching-partitioning framework, they propose two other heuristics called MP and MP$_{\text{LS}}$. By performing extensive experiments, \citet{a1} conclude that the MP$_{\text{LS}}$ algorithm is the best-performing one among the four algorithms, and is also robust against changes in the graph structure.


\citet{7376822} also apply PMMWM to the intermodal transport, and propose a heuristic based on tabu search~\citep{DBLP:journals/informs/Glover89,DBLP:journals/informs/Glover90} and a genetic algorithm~\citep{DBLP:books/daglib/0019083}. They propose three neighborhood structures for the tabu search heuristic and a crossover operator for the genetic algorithm. But these two algorithms are not as effective as the MP$_{\text{LS}}$ algorithm. Therefore, MP$_{\text{LS}}$ is still the best-performing algorithm for the PMMWM. 
% In this work, we select MP$_{\text{LS}}$ as the baseline algorithm, and our proposed MP$_{\text{KM-M}}$ algorithm significantly outperforms MP$_{\text{LS}}$ on the algorithm efficiency while keeping the same effectiveness.
In this work, we proposed FMP\_HEE algorithm significantly outperforms MP$_{\text{LS}}$ both on efficiency and optimality.

==> 13.02-MPLS.tex <==
The MP$_{\text{LS}}$ algorithm~\citep{a1} decomposes the PMMWM problem into two components, i.e., matching and partition. 
% 下文中称为MP框架
Referred to as the MP framework in the following text.
MP$_{\text{LS}}$ is an iterative heuristic algorithm, and each iteration consists of three stages. The first stage generates a maximum matching $\Pi$ of $G = (U,V,E)$, and the second stage calculates a partition $\mathcal{P}$ of $U$ that satisfies constraints (3) and (4) of the problem. Then, the combination of $\mathcal{P}$ and $\Pi$ results in a feasible solution for an input instance. In the third stage, MP$_{\text{LS}}$ makes a slight adjustment on the weight matrix of $E$ and then returns to the first stage of the next iteration, which can help the algorithm to escape from the local optima and find better solutions. We denote $G'$ to be the bipartite graph where the edge weight matrix is adjusted. Starting from $G' = G$, the MP$_{\text{LS}}$ algorithm repeats the three stages until a termination condition is met. Implementation details of the three stages are as follows.

In the first stage, MP$_{\text{LS}}$ applies the KM algorithm~\citep{DBLP:books/daglib/p/Kuhn10} to obtain a minimum weight maximum matching $\Pi$ of the bipartite graph $G'$. %The minimum weight maximum matching 
So match $\Pi$ is a maximum matching such that the total weight of the edges belonging to the matching is minimized.

In the second stage, MP$_{\text{LS}}$ first assumes the maximum matching $\Pi$ of $G'$ is fixed, then the problem can be regarded as a restricted partitioning problem of $U$, by setting the weight of each vertex $u \in U$ to $w_u = c_{uv}, e_{uv} \in \Pi$ (note that when calculating the partition in this stage, $c_{uv}$ is always the original weight of edge $e_{uv}$). MP$_{\text{LS}}$ uses the RPH~\citep{a2} heuristic algorithm to solve the restricted partitioning problem and obtain a feasible solution to the PMMWM.
% 首先生成一个初始解，然后再用局部搜索进行优化
An initial solution is first generated and then optimized with a local search

In the third stage, MP$_{\text{LS}}$ changes the weight of one edge in $G'$ to adjust the bipartite matching solution in the next iteration. Let $k = \mathop{\arg\max_{k \in \{1,...,m\}}{\{\sum_{u \in U_k, e_{uv} \in \Pi}{c_{uv}}\}}}$, then the selected edge $e \in \Pi$ is an edge with the maximum weight among the current edges of $\Pi$ that are incident to vertices of component $U_k$. MP$_{\text{LS}}$ changes the weight of $e$ in $G'$ to a large value ($10^2 c_{\max}$ in default, where $c_{\max}$ is the maximum edge weight in the input graph) to largely reduce the probability that this edge will belong to the matching calculated in the first stage of the next iteration. %, and returns to the first stage.

% The MP$_{\text{LS}}$ algorithm stops when the solution to the PMMWM has not improved for 20 iterations.

==> 16-ConOLD.tex <==
% 我们提出了FIMP-HGA来解决PMMWM问题。The FIMP-HGA adpot the decomposition Match-Partition framework,也用在MP_LS中。在匹配阶段通过增量更新的方式实现精确算法来减少重复计算，将每轮迭代匹配的时间复杂度从$O(n^3)$降至$O(n^2)$。在partition阶段使用genetic algorithm with elite stratege，配合我们提出的Greedy Partition Crossover operator和multi-level local search高效准确的对解空间进行探索，在相同的匹配策略下大幅提升最终解的优度。最后，根据每轮迭代的解动态修改二分图结构保证对解空间的充分搜索。

In this study, we introduced the FIMP-HGA algorithm as a solution to the PMMWM problem, employing the Match-Partition decomposition framework akin to MP$_\text{LS}$. 
%In the match stage, we implemented an exact algorithm through incremental updates to reduce redundant computations, reducing the time complexity per iteration from $O(n^3)$ to $O(n^2)$. 
Notable advancements include the introduction of an exact algorithm during the match stage via incremental updates, reducing time complexity per iteration from $O(n^3)$ to $O(n^2)$.  
%During the partition stage, a hybrid genetic algorithm with an elite strategy is designed, combined with our proposed greedy partition crossover operator and a multi-level local search to explore the solution space efficiently and accurately. This approach significantly enhances the quality of the final solution under the same matching strategy. 
The partition stage features a hybrid genetic algorithm with an elite strategy, complemented by our proposed greedy partition crossover operator and multi-level local search, enhancing solution quality significantly under the same matching strategy. 
%Finally, by dynamically adjusting the bipartite graph structure based on the solution of each iteration, we ensure a thorough search of the solution space.
Finally, dynamic adjustments to the bipartite graph structure  based on the solution of each iteration ensure a thorough exploration of the solution space.

% 实验在提出的4个benchmarks上进行测试，共1750个算例。根据测试结果，FIMP-HGA远远好于the state-of-the-art method. In particular, FIMP-HGA相较于MP-LS，在节约了3-20倍的时间内，运行结果向理论最优解接近了至少90。另外，通过在benchmarks上对FIMP-HGA进行消融测试印证文中提出的各模块对算法的优化效果。最后，通过控制变量法展示了不同特征的算例对算法运行结果的影响。

Our experiments, conducted on four proposed benchmarks encompassing 1750 instances, demonstrate the superiority of FIMP-HGA over the state-of-the-art method. In particular, compared to MP$_\text{LS}$, FIMP-HGA achieves results closer to the theoretical optimum by at least 90\% while reducing computational time by 3-20 times. Additionally, ablation tests on FIMP-HGA validate the optimization effects of the various modules proposed in the study. Lastly, we illustrate the impact of different instance features on algorithm performance in a controlled environment.  

% 在这篇文章的工作中，我们同时从精确和启发式的角度对算法进行优化，大幅改进了解决PMMWM的最优算法。
In this paper, we significantly improve the algorithm for the PMMWM problem through both exact and heuristic optimizations. 
% 在未来的工作中，我们将从如下两个方面继续对该问题进行研究。首先，整理和优化partition stage中提出的hybrid genetic algorithm，尝试应用到相关问题中，如the Multiprocessor Scheduling problem和the Multi-way Number Partition problem. 另外，对于每轮迭代后边的禁忌策略仍有优化空间。相较于integrated方式，decomposed方法没有充分考虑match stage和partition stage的联系。因此可以继续尝试对二分图结构的改动策略，强化这两个stage的联系。
In future work, we plan to continue our research on this problem from two main aspects. Firstly, we aim to refine and optimize the hybrid genetic algorithm proposed for the partition stage and explore its application to related problems, such as the Multiprocessor Scheduling problem and the Multi-way Number Partition problem. 
Additionally, twe acknowledge the potential for improvement in the tabu strategy implemented after each iteration. Compared to the integrated approach, the decomposed method does not fully consider the relationship between the match and partition stages. Therefore, we plan to conduct further  analysis and experimentation aimed at enhancing the interaction between these two stages by adjusting the bipartite graph structure. 

==> 16-Con_OLD.tex <==
% 我们提出了FIMP-HGA来解决PMMWM问题。The FIMP-HGA adpot the decomposition Match-Partition framework,也用在MP_LS中。在匹配阶段通过增量更新的方式实现精确算法来减少重复计算，将每轮迭代匹配的时间复杂度从$O(n^3)$降至$O(n^2)$。在partition阶段使用genetic algorithm with elite stratege，配合我们提出的Greedy Partition Crossover operator和multi-level local search高效准确的对解空间进行探索，在相同的匹配策略下大幅提升最终解的优度。最后，根据每轮迭代的解动态修改二分图结构保证对解空间的充分搜索。

In this study, we introduced the FIMP-HGA algorithm as a solution to the PMMWM problem, employing the Match-Partition decomposition framework akin to MP$_\text{LS}$. 
%In the match stage, we implemented an exact algorithm through incremental updates to reduce redundant computations, reducing the time complexity per iteration from $O(n^3)$ to $O(n^2)$. 
Notable advancements include the introduction of an exact algorithm during the match stage via incremental updates, reducing time complexity per iteration from $O(n^3)$ to $O(n^2)$.  
%During the partition stage, a hybrid genetic algorithm with an elite strategy is designed, combined with our proposed greedy partition crossover operator and a multi-level local search to explore the solution space efficiently and accurately. This approach significantly enhances the quality of the final solution under the same matching strategy. 
The partition stage features a hybrid genetic algorithm with an elite strategy, complemented by our proposed greedy partition crossover operator and multi-level local search, enhancing solution quality significantly under the same matching strategy. 
%Finally, by dynamically adjusting the bipartite graph structure based on the solution of each iteration, we ensure a thorough search of the solution space.
Finally, dynamic adjustments to the bipartite graph structure  based on the solution of each iteration ensure a thorough exploration of the solution space.

% 实验在提出的4个benchmarks上进行测试，共1750个算例。根据测试结果，FIMP-HGA远远好于the state-of-the-art method. In particular, FIMP-HGA相较于MP-LS，在节约了3-20倍的时间内，运行结果向理论最优解接近了至少90。另外，通过在benchmarks上对FIMP-HGA进行消融测试印证文中提出的各模块对算法的优化效果。最后，通过控制变量法展示了不同特征的算例对算法运行结果的影响。

Our experiments, conducted on four proposed benchmarks encompassing 1750 instances, demonstrate the superiority of FIMP-HGA over the state-of-the-art method. In particular, compared to MP$_\text{LS}$, FIMP-HGA achieves results closer to the theoretical optimum by at least 90\% while reducing computational time by 3-20 times. Additionally, ablation tests on FIMP-HGA validate the optimization effects of the various modules proposed in the study. Lastly, we illustrate the impact of different instance features on algorithm performance in a controlled environment.  

% 在这篇文章的工作中，我们同时从精确和启发式的角度对算法进行优化，大幅改进了解决PMMWM的最优算法。
In this paper, we significantly improve the algorithm for the PMMWM problem through both exact and heuristic optimizations. 
% 在未来的工作中，我们将从如下两个方面继续对该问题进行研究。首先，整理和优化partition stage中提出的hybrid genetic algorithm，尝试应用到相关问题中，如the Multiprocessor Scheduling problem和the Multi-way Number Partition problem. 另外，对于每轮迭代后边的禁忌策略仍有优化空间。相较于integrated方式，decomposed方法没有充分考虑match stage和partition stage的联系。因此可以继续尝试对二分图结构的改动策略，强化这两个stage的联系。
In future work, we plan to continue our research on this problem from two main aspects. Firstly, we aim to refine and optimize the hybrid genetic algorithm proposed for the partition stage and explore its application to related problems, such as the Multiprocessor Scheduling problem and the Multi-way Number Partition problem. 
Additionally, twe acknowledge the potential for improvement in the tabu strategy implemented after each iteration. Compared to the integrated approach, the decomposed method does not fully consider the relationship between the match and partition stages. Therefore, we plan to conduct further  analysis and experimentation aimed at enhancing the interaction between these two stages by adjusting the bipartite graph structure. 
